TEASER: Fast and Certifiable Point Cloud Registration

We propose the first fast and certifiable algorithm for the registration of two sets of 3D points in the presence of large amounts of outlier correspondences. We first reformulate the registration problem using a Truncated Least Squares (TLS) cost that is insensitive to a large fraction of spurious correspondences. Then, we provide a general graph-theoretic framework to decouple scale, rotation, and translation estimation, which allows solving in cascade for the three transformations. Despite the fact that each subproblem is still non-convex and combinatorial in nature, we show that (i) TLS scale and (component-wise) translation estimation can be solved in polynomial time via adaptive voting, (ii) TLS rotation estimation can be relaxed to a semidefinite program (SDP) and the relaxation is tight, even in the presence of extreme outlier rates, and (iii) the graph-theoretic framework allows drastic pruning of outliers by finding the maximum clique. We name the resulting algorithm TEASER (Truncated least squares Estimation And SEmidefinite Relaxation). While solving large SDP relaxations is typically slow, we develop a second fast and certifiable algorithm, named TEASER++, that uses graduated non-convexity to solve the rotation subproblem and leverages Douglas-Rachford Splitting to efficiently certify global optimality. For both algorithms, we provide theoretical bounds on the estimation errors, which are the first of their kind for robust registration problems. Moreover, we test their performance on standard, object detection, and the 3DMatch benchmarks, and show that (i) both algorithms dominate the state of the art and are robust to more than 99% outliers, (ii) TEASER++ can run in milliseconds, and (iii) TEASER++ is so robust it can also solve problems without correspondences, where it largely outperforms ICP and it is more accurate than Go-ICP while being orders of magnitude faster.

==> sections/app-proof-cloning.tex <==
%!TEX root = main.tex

\subsection{Proof of~\prettyref{prop:cloning}}
\label{sec:proof:prop:cloning}

% show that solution of one problem can be uniquely  mapped to solution of the other
Here we prove the equivalence between Problem~\eqref{eq:TLSrotation2} and problem~\eqref{eq:TLSrotation4}.
Towards this goal, we show that the latter is simply a reparametrization of the former.

Let us rewrite~\eqref{eq:TLSrotation2} by making the orthogonality constraint $\MR \in \Othree$ explicit 
(recall $\Othree \doteq \setdef{\MR\in\Real{3 \times 3}}{\MR\tran \MR = \eye_3}$): 
\bea
\label{eq:TLSrotationA2}
\min_{
\substack{\MR,
\theta_k, \forall k }} % k=1,\ldots,\nrTIM} 
& \sumAllIM 
 \frac{ (1 + \theta_k) }{ 2 } \frac{  \|  \TIMb_k -  \MR \TIMa_k \|^2 }{  \beta^2_k }  
+ 
\frac{ (1 - \theta_k) }{ 2 } 
\barcsq  \\
\subject 
&
\MR\tran\MR=\eye_3, \;\; \theta_k \in\{-1,+1\}, k=1,\ldots,\nrTIM \nonumber 
\eea
%
% where we also made the constraint $\MR \in \Othree$ explicit. %(recall that $\Othree \doteq \setdef{\MR \in \Real{3\times3}}{\MR\tran\MR=\eye_3}$). 

Noting that the term $\frac{(1 + \theta_k)}{2} \in \{0,1\}$, we can safely move it inside the squared norm and rewrite
eq.~\eqref{eq:TLSrotationA2} as:
%
\bea
\min_{
\substack{\MR, \theta_k, \forall k }} % 
&
\sumAllIM 
\frac{  \| \TIMb - \MR \TIMa 
+ \theta_k \TIMb - \theta_k \MR \TIMa \|^2 }{ 4 \beta^2_k }  
+ 
\frac{ (1 - \theta_k) }{ 2 } 
\barcsq  \label{eq:TLSrotationA3}
\\
\subject 
&
\MR\tran\MR=\eye_3, \;\; \theta_k \in\{-1,+1\}, k=1,\ldots,\nrTIM \nonumber 
\eea
%
Now, we reparametrize the problem by introducing matrices $\MR_k \doteq \theta_k \MR$.
 In particular, we note that these matrices satisfy:
 \bit
 \item $\MR_k\tran \MR_k = (\theta_k\MR)\tran(\theta_k\MR) = \theta_k^2 \eye_3 = \eye_3$ (i.e., $\MR_k \in \Othree$)
 \item $\MR\tran \MR_k = \theta_k \cdot \eye_3 \in \{-\eye_3,+\eye
_3\}$, which also implies 
\item $\theta_k =\ve_1\tran \MR\tran \MR_k\ve_1$, where $\ve_1 \doteq [1 \; 0 \; 0]\tran$.
\eit
These three properties allow writing~\eqref{eq:TLSrotationA3} as:
%
\bea
\min_{
\substack{\MR, \MR_k, \forall k }} % 
&
\sumAllIM 
\frac{  \| \TIMb - \MR \TIMa 
+ \MR\tran \MR_k  \TIMb - \MR_k \TIMa \|^2 }{ 4 \beta^2_k }  
+ 
\frac{ (1 - \ve_1\tran \MR\tran \MR_k \ve_1) }{ 2 } 
\barcsq  \nonumber 
\\
\subject 
\hspace{-5mm}&
\MR\tran\MR=\eye_3, \;\; \MR_k\tran\MR_k=\eye_3,
\nonumber 
 \\
& \MR\tran\MR_k \in\{-\eye,+\eye\},
\; k=1,\ldots,\nrTIM \label{eq:TLSrotationA4}
\eea
%
% where $\ve_1 = [1 \; 0 \; 0]\tran$ and we used the fact that: $\MR\tran \MR_k = \theta_k \cdot \eye_3$, hence for any vector $\vxx$, it holds $\theta_k \vxx = \MR\tran \MR_k \vxx$.
which matches~\eqref{eq:TLSrotation4}, concluding the proof.



% %
% \bea
% \label{eq:TLSrotation3}
% \min_{
% \substack{\MR, \theta_k, \forall k }} % 
% &
% \sumAllIM 
% \frac{  \| (1 + \theta_k) 
% ( \TIMb - \hats \MR \TIMa ) \|^2 }{ 4 \beta^2_k }  
% + 
% \frac{ (1 - \theta_k) }{ 2 } 
% \barcsq 
% \\
% \subject 
% &
%  \theta_k \in\{-1,+1\}
% \eea
% %
%

==> sections/app-remark-noveltyIMs.tex <==
%!TEX root = main.tex

\section{Novelty of \TIMs and \TRIMs}
\label{sec:noveltyIMs}

\LC{add Summary table?}

\begin{remark}[Novelty]
We remark that the idea of using \emph{translation invariant measurements} and \emph{rotation invariant measurements} has been proposed in recent work~\cite{Li19arxiv-fastRegistration,Bustos18pami-GORE,Liu18eccv-registration,agarwal2017icra-RFM-SLAM} while (i) the graph theoretic interpretation of~\prettyref{thm:TIM}
is novel and generalizes previously proposed methods, and (ii) the notion of \emph{translation and rotation invariant measurements} (\TRIMs) is completely new. We also remark that while related work uses invariant measurements 
to filter-out outliers~\cite{Bustos18pami-GORE} or to speed up \bnb~\cite{Li19arxiv-fastRegistration,Liu18eccv-registration}, we show that they also allow computing a \emph{polynomial-time} robust registration solution. 
\end{remark}

==> sections/app-thm-noisyAdversarial-old.tex <==
%!TEX root = ../main.tex

\subsection{Proof of Theorem~\ref{thm:certifiableRegNoisy}}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{theorem}[Estimation Contract with Noisy Inliers and Adversarial Outliers]
% \label{thm:certifiableRegNoisy}
% Assume (i) the set of correspondences contains at least 3 non-collinear and distinct inliers
%  (for an inlier $i$, $\| \vb_i - \sgt \MRgt \va_i - \vtgt \| \leq \beta$, where 
%  $(\sgt, \MRgt, \vtgt)$ denotes the ground truth transformation). 
%  Assume (ii) the inliers belong to the largest set $\calS$  
%  such that for any $i,j \in \calS$, 
%  $| s_{ij} - s | \leq \alpha_{ij}$, 
%  $\| \TIMb_{ij} - s R \TIMa_{ij}\| \leq \beta_{ij}$, 
%  and 
% $\| \vb_{i} - s R \va_{i} - \vt\| \leq \beta_{i}$ 
% for any transformation $(s,\MR,\vt)$.
%  If
%  (iii) the inliers computed by \name (in each subproblem) are such that the sum of their residual error squared is below $\barcsq$, (iv) the rotation subproblem produces a valid certificate 
%  (in the sense of Theorem~\ref{thm:strongDualityNoiseless}), 
%  and (v) \name returns more than $50\%$ inliers, 
% then the output $(\hats, \hatMR, \hatvt)$ of \name satisfies:
% \beq
% |\hats - \sgt| \leq \eta_s, 
% \quad
% \|\hats \hatMR - \sgt \MRgt \| \leq 4 \beta,
% \quad 
% \|\hatvt - \vtgt \| \leq \eta_t
%  \label{item:bounds1}
% \eeq
% where $\eta_s = 2 \max_{ij} \alpha_{ij}$ and $\eta_t = 2\beta + 4\beta \max_i \|\va_{i}\|$. 
%  Moreover, if the scale is know ($\sgt = 1$), the rotation and translation bounds become:
% \beq
% \| \hatMR - \MRgt \| \leq 4 \beta,
% \qquad 
% \|\hatvt - \vtgt \| \leq \LC{???}.
%  \label{item:bounds2}
% \eeq
% \end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Estimation Contract with Noisy Inliers and Adversarial Outliers]
\label{thm:certifiableRegNoisy}
Assume (i) the set of correspondences contains at least 3 non-collinear and distinct inliers,
 where for an inlier $i$, $\| \vb_i - \sgt \MRgt \va_i - \vtgt \| \leq \beta$, and 
 $(\sgt, \MRgt, \vtgt)$ denotes the ground truth transformation. 
 Assume (ii) the outliers do not form a 

 the inliers belong to both 

 belong to the largest set $\calS$  
 such that for any $i,j \in \calS$, 
 $| s_{ij} - s | \leq \alpha_{ij}$, 
 $\| \TIMb_{ij} - s R \TIMa_{ij}\| \leq \beta_{ij}$, 
 and 
$\| \vb_{i} - s R \va_{i} - \vt\| \leq \beta_{i}$ 
for any transformation $(s,\MR,\vt)$.
 If
 (iii) the inliers computed by \name (in each subproblem) are such that the sum of their residual error squared is below $\barcsq$, 
(iv) the rotation subproblem produces a valid certificate 
 (in the sense of Theorem~\ref{thm:strongDualityNoiseless}), 
 and (v) \name returns more than $50\%$ inliers, 
then the output $(\hats, \hatMR, \hatvt)$ of \name satisfies:
\beq
|\hats - \sgt| \leq \eta_s, 
\quad
\|\hats \hatMR - \sgt \MRgt \| \leq 4 \beta,
\quad 
\|\hatvt - \vtgt \| \leq \eta_t
 \label{item:bounds1}
\eeq
where $\eta_s = 2 \max_{ij} \alpha_{ij}$ and $\eta_t = 2\beta + 4\beta \max_i \|\va_{i}\|$. 
 Moreover, if the scale is know ($\sgt = 1$), the rotation and translation bounds become:
\beq
\| \hatMR - \MRgt \| \leq 4 \beta,
\qquad 
\|\hatvt - \vtgt \| \leq \LC{???}.
 \label{item:bounds2}
\eeq
\end{theorem}

We prove Theorem~\ref{thm:certifiableRegNoisy} in two steps. 
First we show that under assumptions (iii)-(iv) of the theorem, the inliers found by \name match the maximum consensus solution. Then, we prove that under assumptions (i)-(ii) the maximum consensus solution is close to the  ground truth, in the sense of inequalities~\eqref{item:bounds1} and~\eqref{item:bounds2} in the theorem. 

\subsubsection{\TLS $\equiv$ \maxCon}
 We prove that solving \TLS for each subproblem leads to the same set of inliers produced by maximum consensus (\maxCon)
 under the 
 assumptions of the theorem. 
 We again denote with $\calM$ the original set of measurements 
 (\ie $\calM = \setOneToN$) and with $\calMIM$ the set of invariant measurements (\ie $\calMIM = \setOneToIM$).

 Let us start with the scale subproblem, where in the presence of noise \TLS and \maxCon take the following form:
 \bit
 \item \TLS scale: $\min_{s} \sumAllIM \min\left( \frac{  (  s-s_k )^2 }{  \alpha^2_k }  \;,\; \barcsq \right)$

 \item \maxCon scale: $\min_{\substack{\calO \subseteq \calMIM \\
 s > 0}} |\calO| 
 \subject 
 |s - s_k| \leq \alpha^2_k\;\; \forall k \in \calMIM \setminus \calO$
 \eit

 TLS achieves cost $\nrOutTLS \barcsq \leq f1tls< (\nrOutTLS+1) \barcsq$ and number of outliers $\nrOutTLS$

 assume by contradiction that MC finds a set with $<\nrOutTLS$ outliers. 

% Condition (ii) in the theorem guarantees that the \MC consensus set contains all the inliers, cost $NoutMC$.
Let us call $\nrOutMC$ the number of outliers detected by a maximum consensus solution.
The \TLS cost computed over the corresponding inlier set, achieves a cost $f\at{1}$ that satisfies 
$NoutMC\barcsq \leq f\at{1} < (NoutMC+1)\barcsq$ 
since the cumulative contribution of the inliers 

If \TLS takes the same set of inliers, it achieves $(NoutMC+1)\barcsq$.

Assume \TLS gets a better solution with cost $fin2 + fout2 <(NoutMC+1)\barcsq$, this solution would have outlier contribution $fout2 < (NoutMC+1)\barcsq - fin2 < NoutMC\barcsq$ (since $fin2<\barcsq$), hence $<NoutMC$ outliers contradicting optimality of MC.


 % Assume the inliers computed by \name have cumulative residual error $<\barcsq$ (condition (iii) in the theorem).
 % Then the cost achieved by the \TLS scale estimation at its optimal estimate $\hats$ is $<\barcsq + \nrOutTLS \barcsq = (\nrOutTLS+1) \barcsq$ where the term $\barcsq$ is the contribution of the inliers to the cost, while $\nrOutTLS \barcsq$ is the contribution to the outliers (as in the previous proofs, $\nrOutTLS$ is the number of 
 % outliers returned by Algorithm~\ref{alg:adaptiveVoting}). % in Section~\ref{sec:scaleEstimation}. 
 % Now assume by contradiction, that maximum consensus  finds a better solution $s_\maxCon$ with $\nrOutMC < \nrOutTLS$ outliers. Then, the solution $s_\maxCon$ 
 % %corresponds to a choice of $(s, \vt, \MR)$ that 
 % makes 
 % $N-\nrOutMC$ residuals in $[0,\alpha^2_k]$, while introducing at most $\nrOutMC$ outliers. Such an estimate would achieve a \TLS cost of at most $\nrOutMC < \nrOutTLS$, contradicting the optimality of $\hats$. 
 The same logic applies to the rotation and translation subproblems, leading to identical conclusions 
 under the assumption that the rotation subproblem finds a certifiably optimal estimate (condition (iv) in the theorem).  
 
% \LC{with Hank we proved this by assuming that every LS solution over any consensus set has error below $\barcsq$, a pretty bad condition. I have the gut feeling that if we assume that the \TLS inliers are $>50\%$ and we ensure that these inliers are separated from the outliers, we can prove this}
 % Assume the inliers computed by \name are such that the sum of their residual error squared is below $\barcsq$ 
 % (condition (iii) in the theorem).
 % Then the cost achieved by the \TLS scale estimation at its optimal estimate $\hats$ is 
 % $f_s < \barcsq + \nrOutTLS \barcsq$ (the first summand follows from the fact that the inlier residuals are bounded by $\barc$), where $\nrOutTLS$ is the number of 
 % outliers returned by the algorithm in Section~\ref{sec:scaleEstimation}. 
 % Now assume by contradiction, that maximum consensus finds a better solution $s_\maxCon$ with $\nrOutMC < \nrOutTLS$ outliers. Then, the solution $s_\maxCon$ 
 % %corresponds to a choice of $(s, \vt, \MR)$ that 
 % makes 
 % $N-\nrOutMC$ residuals equal to zero, while introducing at most $\nrOutMC$ outliers. Such an estimate would achieve a \TLS cost of at most $\nrOutMC < \nrOutTLS$, contradicting the optimality of $\hats$. 
 % The same logic applies to the rotation and translation subproblems, leading to identical conclusions 
 % under the assumption that the rotation subproblem finds a certifiably optimal estimate (condition (iv)).  
 

\subsubsection{Noisy recovery of maximum consensus} We now prove that maximum consensus produces a solution ``close'' to the ground truth under the assumptions of the theorem. Let us start with the scale subproblem. 
Assumption (ii) in the theorem ensures that the maximum consensus set contains all inliers in each subproblem.
Let us now derive the bounds on the resulting estimate, starting from the scale estimation.
Since the scale estimation selects all the inliers, plus potentially some outliers, it holds for some of the 
selected measurements $i,j$:
\bea
|\sgt - \hats | = |\sgt - \hats + \eps^s_{k} - \eps^s_{k} | \\
 \overset{(a)}{\leq}  |\sgt + \eps^s_{k} - \hats| + |\eps^s_{k} | \\
 \overset{(b)}{\leq}  | s_{k} - \hats |  - \alpha_{ij}   \overset{(c)}{\leq} 2 \alpha_{ij} 
\eea
where in (a) we used the triangle inequality, in (b) we noticed that for inliers $i,j$, it holds 
$|\eps^s_{k}| \leq \alpha_{ij}$ and $\sgt + \eps^s_{k} = s_k$, and in (c) we noticed that for $s_k$ to be 
considered an inlier by \TLS, $| s_{k} - \hats | \leq \alpha_{ij}$.
Since the inequality has to hold for all the true inliers, but
we do not know which ones of the measurements selected by \TLS are true inliers, we substitute the bound with:
\bea
|\sgt - \hats |  \leq 2 \max_{ij} \alpha_{ij}
\eea
which proves the first bound in~\eqref{item:bounds1}, with $\eta_s \doteq 2 \max_{ij} \alpha_{ij}$.





Let us now move to rotation estimation. 
Since the rotation estimation also selects all the inliers, plus potentially some outliers, it holds for some of the selected measurements $i,j$:
\bea
\| \sgt \MRgt \TIMa_{ij} - \hats \hatMR \TIMa_{ij} \|  = 
\| \sgt \MRgt \TIMa_{ij} - \hats \hatMR \TIMa_{ij} + \veps_{ij} -\veps_{ij}  \| \\
 \overset{(a)}{=}
\| \TIMb_{ij}- \hats \hatMR \TIMa_{ij}  -\veps_{ij}  \| \\
 \overset{(b)}{\leq}
\| \TIMb_{ij} - \hats \hatMR \TIMa_{ij} \|  + \| \veps_{ij}  \|
 \overset{(c)}{\leq} 2 \TIMNoiseBound_{ij} = 4 \beta
\eea
where in (a) we noted that noticed that for inliers $i,j$, $\TIMb_{ij} = \sgt \MRgt \TIMa_{ij} + \veps_{ij}$, 
in (b) we used the triangle inequality, and in (c) we noticed 
that it holds 
$|\veps_{ij}| \leq \TIMNoiseBound_{ij}$ and that for $(i,j)$ to be 
considered an inlier by \TLS, $\| \TIMb_{ij}- \hats \hatMR \TIMa_{ij} \| \leq \TIMNoiseBound_{ij}$. 
Since the inequality has to hold for all the true inliers, but
we do not know which ones of the measurements selected by \TLS are true inliers, we substitute the bound with:
\bea
\label{eq:rotBound}
\| \sgt \MRgt \TIMa_{ij} - \hats \hatMR \TIMa_{ij} \|  \leq 2 \max_{ij} \TIMNoiseBound_{ij} = 4 \beta
\eea
since we assumed all inliers have noise $\|\veps_i\| \leq \beta$ and $\|\veps_{ij}\| \leq 2\beta$. This proves the second bound in~\eqref{item:bounds1}.
  




We can use a similar proof strategy for the translation case.
 Since the translation estimation also selects all the inliers, it holds for some of the selected measurement $i$:
\bea
\| \vtgt - \hatvt \|  
\nonumber  \\
= \| \vtgt \!-\! \hatvt + (\sgt \MRgt \va_{i} \!-\! \hats \hatMR \va_{i}) \!-\! (\sgt \MRgt \va_{i} \!-\! \hats \hatMR \va_{i})
\!+\! \veps_i \!-\! \veps_i \|  
\nonumber  \\
= \| (\sgt \MRgt \va_{i} \!+\! \vtgt \!+\! \veps_i) \!-\! \hatvt \!-\! \hats \hatMR \va_{i} \!-\! (\sgt \MRgt \va_{i} \!-\! \hats \hatMR \va_{i})
\!-\! \veps_i \|
\nonumber  \\
 \overset{(a)}{=} \| \vb_{i} \!-\! \hatvt \!-\! \hats \hatMR \va_{i} \!-\! (\sgt \MRgt \va_{i} \!-\! \hats \hatMR \va_{i})
\!-\! \veps_i \| 
\nonumber  \\
 \overset{(b)}{\leq} \| \vb_{i} \!-\! \hatvt \!-\! \hats \hatMR \va_{i} \| + 
 \| \sgt \MRgt \va_{i} \!-\! \hats \hatMR \va_{i} \| + \| \veps_i \| 
 \nonumber  \\
  \overset{(c)}{\leq} 2\beta + 
 \| \sgt \MRgt \va_{i} \!-\! \hats \hatMR \va_{i} \| 
 \overset{(d)}{\leq} 2\beta + 
 \| \sgt \MRgt  \!-\! \hats \hatMR  \| \|\va_{i}\|  
 \nonumber  \\
  \overset{(e)}{\leq} 2\beta + 4\beta \|\va_{i}\| \nonumber  
\eea
where in (a) we noticed that for an inlier $i$, $\vb_{i} = \sgt \MRgt \va_{i} + \veps_{i}$, 
in (b) we used the triangle inequality, 
in (c) we used that for inliers $|\veps_{i}| \leq \beta$ and that for $i$ to be 
considered an inlier by \TLS, $\| \vb_{i}- \hats \hatMR \va_{i}-\hatvt \| \leq \beta$,
in (d) we used the sub-multiplicativity of  the matrix-vector product, 
in (e) we used the rotation bound in~\eqref{eq:rotBound}.
Since the inequality has to hold for all the true inliers, but
we do not know which ones of the measurements selected by \TLS are true inliers, we substitute the bound with:
\bea
\| \vtgt - \hatvt \| \leq 2\beta + 4\beta \max_i \|\va_{i}\| \doteq \eta_t
\eea
which proves the third bound in~\eqref{item:bounds1}.
% \LC{this bound is very loose - I believe it can be improved to be $2\beta$ or close.}
% \bea
% \| \vtgt - \hatvt \|  \\
% = \| \vb_i - \sgt \MRgt \va_{i} - \eps_i  - \hatvt \|
% \eea

Let us now focus on the case with known scale and let us derive the bounds in~\eqref{item:bounds2}.
The first bound is trivial to prove since it is a particularization of 
the bound
$\|\hats \hatMR - \sgt \MRgt \| \leq 4 \beta$ (already proven in the unknown scale case), to the 
case where the scale is known ($\hats = \sgt = 1$).
% The second bound is less trivial and we prove it below.
For the translation, instead, we  adopt a different proof strategy to obtain a stronger bound.
%derive a stronger bound compared to the one in 

==> sections/experiments-multipleObjects.tex <==
%!TEX root = ../main.tex

\subsection{Experiments with Multiple Identical Objects}
\label{sec:multipleObjects}

\LC{
Extensions:
-	Multiple objects
o	Multiple cliques
o	Quaternion-based formulation catches multiple objects
}

==> sections/fig-benchmarkUnknownScale.tex <==
%!TEX root = main.tex

\begin{figure}[h]
	\begin{center}
	\begin{minipage}{\textwidth}
	\hspace{-0.2cm}
	\begin{tabular}{ccc}%
		\myhspace
			\begin{minipage}{3cm}%
			\centering%
			\includegraphics[width=\columnwidth]{scale_err_unknown_scale_ss.pdf} \\
			(a) Scale error
			\end{minipage}
		& 
		\myhspace
			\begin{minipage}{3cm}%
			\centering%
			\includegraphics[width=\columnwidth]{rot_err_unknown_scale_ss.pdf} \\
			(b) Rotation error
			\end{minipage}
			& 
			\myhspace
			\begin{minipage}{3cm}%
			\centering%
			\includegraphics[width=\columnwidth]{trans_err_unknown_scale_ss.pdf} \\
			(c) Translation error
			\end{minipage}
		\end{tabular}
	\end{minipage}
	\begin{minipage}{\textwidth}
	\end{minipage}
	\vspace{-3mm} 
	\caption{Benchmark results for registration with unknown scale.
	 \label{fig:benchmarkUnknownScale}}
	\vspace{-8mm} 
	\end{center}
\end{figure}

==> sections/fig-overview-backup.tex <==
%!TEX root = ../main.tex

\newcommand{\myhspace}{\hspace{-2mm}}
\newcommand{\myvspace}{\hspace{-4mm}}
\newcommand{\mpwt}{2.8cm}
\newcommand{\mpw}{4cm}

\begin{figure}[t!]
	\begin{center}
	\begin{minipage}{\textwidth}
	\begin{tabular}{ccc}%
		\myhspace
			\begin{minipage}[t][][t]{\mpwt}%
			\centering%
			\includegraphics[width=1\columnwidth]{front_page/fp_corrs_1.png} \myvspace\\
			(a) with correspondences %(99\% outlier rate)
			\end{minipage}
		& \myhspace
			\begin{minipage}[t][][t]{\mpwt}%
			\centering%
			\includegraphics[width=0.9\columnwidth]{front_page/fp_corrs_ransac_cropped.png} \myvspace\\
			(b) \ransac 
			\end{minipage}
		& \myhspace
			\begin{minipage}[t][][t]{\mpwt}%
			\centering%
			\includegraphics[width=0.9\columnwidth]{front_page/fp_corrs_tpp_cropped.png} \myvspace\\
			(c) \namepp %(green dots indicate the inliers selected by \namepp)
			\end{minipage}
		\\
		\myhspace
			\begin{minipage}[t][][t]{\mpwt}%
			\centering%
			\includegraphics[width=0.9\columnwidth]{front_page/fp_bf_1} \myvspace\\
			(d) without correspondences %(50\% overlap)
			\end{minipage}
		& \myhspace
			\begin{minipage}[t][][t]{\mpwt}%
			\centering%
			\includegraphics[width=0.9\columnwidth]{front_page/fp_bf_icp} \myvspace\\
			(e) \ICP
			\end{minipage}
		& \myhspace
			\begin{minipage}[t][][t]{\mpwt}%
			\centering%
			\includegraphics[width=0.77\columnwidth]{front_page/fp_bf_tpp} \myvspace\\
			(f) \namepp
			\end{minipage}
		\end{tabular}
		\\
	\begin{tabular}{p{0.5cm}p{\mpw}p{\mpw}}%
	% ================================================================
		\begin{minipage}{0.5cm}%
		\rotatebox{90}{Object Localization}
		\end{minipage}
		& \hspace{-5mm}
			\begin{minipage}{\mpw}%
			\centering%
			\includegraphics[trim= 20mm 0mm 20mm 0mm, clip, width=1.0\columnwidth]{scene_3_a_5.pdf} \myvspace\\
			(g) Correspondences
			\end{minipage}
		& \hspace{-8mm}
			\begin{minipage}{\mpw}%
			\centering%
			\includegraphics[trim= 20mm 0mm 20mm 0mm, clip,width=1.0\columnwidth]{scene_3_c_5.pdf} \myvspace\\
			(h) \namepp
			\end{minipage}
	% ================================================================
			\\
		\begin{minipage}{0.5cm}%
		\rotatebox{90}{Scan Matching}
		\end{minipage}
		& \hspace{-5mm}
			\begin{minipage}{\mpw}%
			\centering%
			\includegraphics[width=0.95\columnwidth]{front_page/fp_scanmatching_2_1_thicker} \myvspace\\
			(j) Correspondences
			\end{minipage}
		& \hspace{-8mm}
			\begin{minipage}{\mpw}%
			\centering%
			\includegraphics[width=1.0\columnwidth]{front_page/fp_scanmatching_2_2} \myvspace\\
			(k) \namepp
			\end{minipage}
	\end{tabular}
	\end{minipage}
	\vspace{-3mm} 
	\caption{
	We address 3D registration in the realistic case where 
	many point-to-point correspondences are outliers due to incorrect matching.
	(a) \bunny dataset (source cloud in blue and target cloud in red) with 99\% outliers (shown as magenta points) and 5\% inliers (shown as green lines). 
	Existing algorithms, such as \ransac (b), can produce largely incorrect estimates without notice even after running for 10,000 iterations.
	Our certifiable algorithms largely outperform the state of the art in 
	terms of robustness and accuracy, and a fast implementation, named \namepp (c), computes accurate estimates in milliseconds event with extreme outlier rates %(\eg 99\% of the correspondences are outliers) 
	and finds the small set of inliers (shown as green dots).
	The unprecedented robustness of \namepp enables the solution of correspondence-free registration problems (d), where \ICP (e) fails without a good initial guess, while our \namepp (d) succeeds without need for an initial guess. We test our approach in challenging object localization (f-g) and scan matching (j-k) RGB-D dataset, using both traditional features (\ie FPFH~\cite{Rusu09icra-fast3Dkeypoints}) and deep-learned features (\ie~3DSmoothNet~\cite{gojcic19cvpr-3dsmoothnet}).
	%The algorithm also outperforms deep learning methods in realistic problems (e)-(f).
	 \label{fig:overview}\vspace{-0.7cm}}
	\end{center}
\end{figure}

==> sections/futureWork.tex <==
%!TEX root = ../main.tex

\section{Future Work and Opportunities}

\bit
\item explore all cliques
\item multiple objects
\item improve feature detection and correspondences
\eit

==> sections/guarantee-noisy-old.tex <==
%!TEX root = ../main.tex

\subsubsection{Noisy Case}
\label{sec:guaranteesNoisy}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Estimation Contract with Noisy Inliers and Adversarial Outliers]
\label{thm:certifiableRegNoisy}
Assume (i) the set of correspondences contains at least 3 non-collinear and distinct inliers
 (for an inlier $i$, $\| \vb_i - \sgt \MRgt \va_i - \vtgt \| \leq \beta$, where 
 $(\sgt, \MRgt, \vtgt)$ denotes the ground truth transformation). 
 Assume (ii) the inliers belong to the largest set $\calS$  
 such that for any $i,j \in \calS$, 
 $| s_{ij} - s | \leq \alpha_{ij}$, 
 $\| \TIMb_{ij} - s R \TIMa_{ij}\| \leq \beta_{ij}$, 
 and 
$\| \vb_{i} - s R \va_{i} - \vt\| \leq \beta_{i}$ 
for any transformation $(s,\MR,\vt)$.
 % $\{i \in \{1,\ldots,N\} : \vb_i = s \MR \va_i + \vt, \forall (s, \MR, \vt)\}$.
 %  and (iii) the outliers are in \emph{generic position} (\eg they are perturbed by random noise).
 If
 (iii) the inliers computed by \name (in each subproblem) are such that the sum of their residual error squared is below $\barcsq$, and (v) the rotation subproblem produces a valid certificate 
 (in the sense of Theorem~\ref{thm:certifiableRotationEstimation}), 
then the output $(\hats, \hatMR, \hatvt)$ of \name satisfies:
\ben
\item $|\hats - \sgt| \leq \eta_s$ \label{item:scale}
\item $\|\hats \hatMR - \sgt \MRgt \| \leq 4 \beta$ \label{item:rot}
\item $\|\hatvt - \vtgt \| \leq \eta_t$ \label{item:tran}
\een
where $\eta_s = 2 \max_{ij} \alpha_{ij}$ and $\eta_t = 2\beta + 4\beta \max_i \|\va_{i}\|$. 
\LC{Moreover, if the scale is know (say $\sgt = 1$), the rotation and translation bounds simplify to:
$\| \hatMR - \MRgt \| \leq 4 \beta$ and $\|\hatvt - \vtgt \| \leq ???$.}
% Moreover, all outliers such that $\| \vb_i - \sgt \MRgt \va_i - \vtgt \| \geq \red{??}$ are rejected by \name.
\end{theorem}

\begin{proof}
We prove Theorem~\ref{thm:certifiableRegNoisy} in two steps. 
First we show that under assumptions (iii)-(iv) of the theorem, the inliers found by \name match the maximum consensus solution. Then, we prove that under assumptions (i)-(ii) the maximum consensus solution is close to the  ground truth, in the sense of inequalities~\ref{item:scale}-\ref{item:tran} in the theorem. 

\myparagraph{\TLS $\equiv$ maximum consensus}
 We prove that solving \TLS for each subproblem leads to the same set of inliers produced by maximum consensus 
 under the 
 assumptions of the theorem. 
 For notational convenience we again denote with $\calM$ the original set of measurements 
 (\ie $\calM = \setOneToN$) and with $\calMIM$ the set of invariant measurements (\ie $\calMIM = \setOneToIM$).

 Let us start with the scale subproblem, where in the presence of noise \TLS and \maxCon take the form:
 \bit
 \item \TLS scale: $\min_{s} \sumAllIM \min\left( \frac{  (  s-s_k )^2 }{  \alpha^2_k }  \;,\; \barcsq \right)$

 \item \maxCon scale: $\min_{\substack{\calO \subseteq \calMIM \\
 s > 0}} |\calO| 
 \subject 
 |s - s_k| \leq \alpha^2_k \forall k \in \calMIM \setminus \calO$
 \eit

\LC{with Hank we proved this by assuming that every LS solution over any consensus set has error below $\barcsq$, a pretty bad condition. I have the gut feeling that if we assume that the \TLS inliers are $>50\%$ and we ensure that these inliers are separated from the outliers, we can prove this}
 % Assume the inliers computed by \name are such that the sum of their residual error squared is below $\barcsq$ 
 % (condition (iii) in the theorem).
 % Then the cost achieved by the \TLS scale estimation at its optimal estimate $\hats$ is 
 % $f_s < \barcsq + \nrOutTLS \barcsq$ (the first summand follows from the fact that the inlier residuals are bounded by $\barc$), where $\nrOutTLS$ is the number of 
 % outliers returned by the algorithm in Section~\ref{sec:scaleEstimation}. 
 % Now assume by contradiction, that maximum consensus finds a better solution $s_\maxCon$ with $\nrOutMC < \nrOutTLS$ outliers. Then, the solution $s_\maxCon$ 
 % %corresponds to a choice of $(s, \vt, \MR)$ that 
 % makes 
 % $N-\nrOutMC$ residuals equal to zero, while introducing at most $\nrOutMC$ outliers. Such an estimate would achieve a \TLS cost of at most $\nrOutMC < \nrOutTLS$, contradicting the optimality of $\hats$. 
 % The same logic applies to the rotation and translation subproblems, leading to identical conclusions 
 % under the assumption that the rotation subproblem finds a certifiably optimal estimate (condition (iv)).  
 

\myparagraph{Noisy recovery of maximum consensus} We now prove that maximum consensus produces a solution ``close'' to the ground truth under the assumptions of the theorem. Let us start with the scale subproblem. 
Assumption (ii) in the theorem ensures that the maximum consensus set contains all inliers in each subproblem.
Let us now derive the bounds on the resulting estimate, starting from the scale estimation.
Since the scale estimation selects all the inliers, plus potentially some outliers, it holds for some of the 
selected measurements $i,j$:
\bea
|\sgt - \hats | = |\sgt - \hats + \eps^s_{k} - \eps^s_{k} | \\
 \overset{(a)}{\leq}  |\sgt + \eps^s_{k} - \hats| + |\eps^s_{k} | \\
 \overset{(b)}{\leq}  | s_{k} - \hats |  - \alpha_{ij}   \overset{(c)}{\leq} 2 \alpha_{ij} 
\eea
where in (a) we used the triangle inequality, in (b) we noticed that for inliers $i,j$, it holds 
$|\eps^s_{k}| \leq \alpha_{ij}$ and $\sgt + \eps^s_{k} = s_k$, and in (c) we noticed that for $s_k$ to be 
considered an inlier by \TLS, $| s_{k} - \hats | \leq \alpha_{ij}$.
Since the inequality has to hold for all the true inliers, but
we do not know which ones of the measurements selected by \TLS are true inliers, we substitute the bound with:
\bea
|\sgt - \hats |  \leq 2 \max_{ij} \alpha_{ij}
\eea
which proves the first bound, with $\eta_s \doteq 2 \max_{ij} \alpha_{ij}$.

Let us now move to rotation estimation. 
Since the rotation estimation also selects all the inliers, plus potentially some outliers, it holds for some of the selected measurements $i,j$:
\bea
\| \sgt \MRgt \TIMa_{ij} - \hats \hatMR \TIMa_{ij} \|  = 
\| \sgt \MRgt \TIMa_{ij} - \hats \hatMR \TIMa_{ij} + \eps_{ij} -\eps_{ij}  \| \\
 \overset{(a)}{=}
\| \TIMb_{ij}- \hats \hatMR \TIMa_{ij}  -\eps_{ij}  \| \\
 \overset{(b)}{\leq}
\| \TIMb_{ij} - \hats \hatMR \TIMa_{ij} \|  + \| \eps_{ij}  \|
 \overset{(c)}{\leq} 2 \beta_{ij} = 4 \beta
\eea
where in (a) we noted that noticed that for inliers $i,j$, $\TIMb_{ij} = \sgt \MRgt \TIMa_{ij} + \eps_{ij}$, 
in (b) we used the triangle inequality, and in (c) we noticed 
that it holds 
$|\eps_{ij}| \leq \beta_{ij}$ and that for $(i,j)$ to be 
considered an inlier by \TLS, $\| \TIMb_{ij}- \hats \hatMR \TIMa_{ij} \| \leq \beta_{ij}$. 
Since the inequality has to hold for all the true inliers, but
we do not know which ones of the measurements selected by \TLS are true inliers, we substitute the bound with:
\bea
\label{eq:rotBound}
\| \sgt \MRgt \TIMa_{ij} - \hats \hatMR \TIMa_{ij} \|  \leq 2 \max_{ij} \beta_{ij} = 4 \beta
\eea
since we assumed all inliers have noise $\|\eps_i\| \leq \beta$. This proves the second bound in the theorem.
  
We can use a similar proof strategy for the translation case.
 Since the translation estimation also selects all the inliers, it holds for some of the selected measurement $i$:
\bea
\| \vtgt - \hatvt \|    \\
= \| \vtgt \!-\! \hatvt + (\sgt \MRgt \va_{i} \!-\! \hats \hatMR \va_{i}) \!-\! (\sgt \MRgt \va_{i} \!-\! \hats \hatMR \va_{i})
\!+\! \eps_i \!-\! \eps_i \|  \\
= \| (\sgt \MRgt \va_{i} \!+\! \vtgt \!+\! \eps_i) \!-\! \hatvt \!-\! \hats \hatMR \va_{i} \!-\! (\sgt \MRgt \va_{i} \!-\! \hats \hatMR \va_{i})
\!-\! \eps_i \| \\
 \overset{(a)}{=} \| \vb_{i} \!-\! \hatvt \!-\! \hats \hatMR \va_{i} \!-\! (\sgt \MRgt \va_{i} \!-\! \hats \hatMR \va_{i})
\!-\! \eps_i \| \\
 \overset{(b)}{\leq} \| \vb_{i} \!-\! \hatvt \!-\! \hats \hatMR \va_{i} \| + 
 \| \sgt \MRgt \va_{i} \!-\! \hats \hatMR \va_{i} \| + \| \eps_i \| \\
  \overset{(c)}{\leq} 2\beta + 
 \| \sgt \MRgt \va_{i} \!-\! \hats \hatMR \va_{i} \| 
 \overset{(d)}{\leq} 2\beta + 
 \| \sgt \MRgt  \!-\! \hats \hatMR  \| \|\va_{i}\|   \\ 
  \overset{(e)}{\leq} 2\beta + 4\beta \|\va_{i}\|
\eea
where in (a) we noted that noticed that for an inlier $i$, $\vb_{i} = \sgt \MRgt \va_{i} + \eps_{i}$, 
in (b) we used the triangle inequality, 
in (c) we used that for inliers $|\eps_{i}| \leq \beta$ and that for $i$ to be 
considered an inlier by \TLS, $\| \vb_{i}- \hats \hatMR \va_{i}-\hatvt \| \leq \beta$,
in (d) we used the sub-multiplicativity of  the matrix-vector product, 
in (e) we used the rotation bound in~\eqref{eq:rotBound}.
Since the inequality has to hold for all the true inliers, but
we do not know which ones of the measurements selected by \TLS are true inliers, we substitute the bound with:
\bea
\| \vtgt - \hatvt \| \leq 2\beta + 4\beta \max_i \|\va_{i}\| = \eta_t
\eea
which proves the third bound in the theorem.
\LC{this bound is very loose - I believe it can be improved to be $2\beta$ or close.}
% \bea
% \| \vtgt - \hatvt \|  \\
% = \| \vb_i - \sgt \MRgt \va_{i} - \eps_i  - \hatvt \|
% \eea
\end{proof}


==> sections/old/experiments_old.tex <==
%!TEX root = main.tex

\section{Experiments and Applications}
\label{sec:experiments}


In all the following experiments, $\bar{c}^2=1$ for scale, rotation and translation estimation.
\subsection{Test of Scale, Rotation, Translation and Maximal Clique Inlier Selection Solvers}
\label{sec:separateSolver}
We first test the scale, rotation, translation and maximal clique inlier selection (MCIS) solvers separately to evaluate their robustness against increasing outlier rates. For this test, we use the \emph{bunny} point cloud dataset from Stanford 3D Scanning Repository~\cite{Curless96siggraph} and resize the point cloud to be within a $[0,1]^3$ unit cube.

{\bf Scale Solver.} The bunny is first downsampled to $N=50$ points, and then a random transformation $(s, \MR, \vt)$ is applied according to Eq.~\eqref{eq:robustGenModel} where $1\leq s \leq 5$ and $\Vert \vt \Vert \leq 1$. To generate the unknown but bounded noise $\veps_i$, we first sample $\veps_i \sim \calN(\bm{0},\sigma^2 \MI)$, if the norm $\Vert \veps_i \Vert$ is larger than the bound $\beta_i=\beta$, we resample $\veps_i$ until its norm is smaller than $\beta$, where we assume all measurements share the same noise distribution and noise bound. $\sigma$ is set to be 0.01 to test low noise regime. Because $\veps_i \sim \calN(\bm{0},\sigma^2 \MI)$, the square of the norm $\Vert \veps_i \Vert^2$ follows a Chi-square distribution with 3 degrees of freedom: $\frac{\Vert \veps_i \Vert^2}{\sigma^2} \sim \chi^2(3)$. Hence we set $\beta$ such that $\mathbb{P}\left(\frac{\Vert \veps_i \Vert^2}{\sigma^2} < \beta \right) > p$ and $p=99.9999\%$ is chosen to be conservative about the bound. To generate outliers, we randomly choose a scalar between 0 and 5, multiply the scalar by a random unit vector (direction) and use them to replace the correct inliers. Increasing outlier ratios of $\{0,0.2,0.4,0.6,0.7,0.8,0.9\}$ are chosen and 40 runs of experiments are performed for each outlier level. Given the two point clouds with noise and outliers simulated above, the scale solver first creates $N(N-1)$ TIMs according to the fully connected graph and uses the adaptive voting algorithm to solve for the scale. We compute both "Maximum consensus" and "TLS" estimates of the scale and compare their performance. Fig.~\ref{fig:benchmark_separate_solvers}(a) shows box plots of the scale error with increasing outlier ratios. It can be observed that "TLS" scale solver is robust against 80\% outlier ratio, while "Maximum consensus" scale solver is robust against 70\% outlier ratio, though there are only three failures at 80\% outlier level.


%%%%%%%%%%%%%%%%%%%%%%%%%
\input{fig-benchmark_separate_solvers}
%%%%%%%%%%%%%%%%%%%%%%%%%

{\bf Rotation Solver.} To test the rotation solver, the bunny is first downsampled to $N=50$ points, and then only a random rotation $\MR$ is applied while the scale is set to 1 and the translation is set to zero. The same method as in testing the scale solver is used to generate noise and outliers, and same outlier levels and number of runs per outlier level are used. Rotation error and stable rank are boxplotted in Fig.~\ref{fig:benchmark_separate_solvers}(b). One can see that the rotation SDP solver is robust up to 90\% outliers, with stable rank being close to 3 and low rotation error.

{\bf Translation Solver.} Testing condition of translation solver is same as rotation solver, except that only a random translation $vt$ is applied to the downsampled bunny point cloud. Component-wise translation estimation using both "Maximum consensus" and "TLS" solvers are performed and Fig.~\ref{fig:benchmark_separate_solvers}(c) demonstrates the robustness of "TLS" solver against 80\% outliers and the robustness of "Maximum consensus" solver against 70\% outliers, similar to what has been seen in the scale solver test.

{\bf Maximal Clique Inlier Selection Solver.} In this test, we downsample bunny dataset to $N=1000$ and fix scale $s=1$ when applying the random transformation. The Maximal Clique Inlier Selection (MCIS) solver first removes outlier TRIMs, then uses the algorithm in~\cite{Eppstein10isac-maxCliques} to find all the maximal cliques in the remaining graph $(\calV,\calE')$, and returns the maximal clique with maximum cardinality (MCMC). We use the grouth truth to calculate the inlier ratio in MCMC and compare it with the original inlier ratio, as shown in Fig.~\ref{fig:benchmark_separate_solvers}. We find that among all the simulations (40 runs per outlier level as before), there is only one case at 90\% outlier ratio where the MCMC returned by MCIS contains all outliers, which are pair-wise scale consistent. However, we comment that this can be easily resolved because if MCIS returns an MCMC that contains all outliers, the rotation SDP with not be tight and the algorithm can go back and select the second largest MCMC. 

\subsection{Benchmark \name}
\label{sec:benchmark}
We benchmark \name against two state-of-the-art robust registration techniques: Fast Global Registration (\FGR)~\cite{Zhou16eccv-fastGlobalRegistration} and Guaranteed Outlier Removal (\GORE)~\cite{Bustos18pami-GORE} under increasing outlier ratios $\{0,0.2,0.4,0.6,0.7,0.8,0.9\}$. In addition, we also run registration using two standard RANSAC schemes: one RANSAC with maximum iterations 1,000 (\ransaconek) and the other RANSAC with timeout 60s (\ransac). Four point cloud datasets, \emph{bunny}, \emph{armadillo}, \emph{dragon} and \emph{buddha}, from the Stanford 3D Scanning Repository are selected and downsampled to $N=100$ for synthetic experiments.

%%%%%%%%%%%%%%%%%%%%%%%%%
\input{fig-benchmark}
%%%%%%%%%%%%%%%%%%%%%%%%%

{\bf Known Scale.} We first perform the benchmark with known scale $s=1$ and only transform the point cloud with random rotation and translation. Noise and outliers are generated as in \prettyref{sec:separateSolver}, and 40 experiments are carried out for each outlier level. Fig.~\ref{fig:benchmak} \todo.

{\bf Unknown Scale.} When the scale is unknown, since GORE is unable to solve scale, we only benchmark \name against \FGR (although the original algorithm in~\cite{Zhou16eccv-fastGlobalRegistration} did not solve scale, we extend it by using Horn's method to solve scale during each iteration), \ransaconek and \ransac. Fig.~\ref{fig:benchmarkUnknownScale} plots the scale, rotation and translation error under increasing outlier level $\{0.6,0.7,0.8,0.9\}$, and we comment that all methods perform well when the outlier ratio is below 60\%. \FGR has the lowest breakdown point at 70\%, while \ransaconek and \name can afford up to 80\% outlier ratio. Although \ransac with 60s timeout outperforms global methods at 90\% outlier rate, it requires 100K or even more iterations to converge, which is not practical for real applications.

%%%%%%%%%%%%%%%%%%%%%%%%%
%\input{fig-benchmarkUnknownScale}
%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Benchmark \name under Extreme Outlier Rates}
\label{sec:benchmarkExtreme}
Motivated by the fact that over 95\% of the correspondences generated by 3D keypoint matching methods can be outliers, we further benchmark the performance of \name under extreme outlier rates from 95\% to 99\% with known scale and $N=1000$ correspondences. Fig.~\ref{fig:benchmark_extreme_outlier} shows the boxplots of rotation error and translation error. Both \name and GORE are robust against up to 99\% outliers, while RANSAC with 60s timeout can resist 98\% outliers with about $10^6$ iterations. RANSAC with $10^4$ iterations and FGR perform badly under extreme outlier ratios. It is worth notice that though both GORE and \name are robust against extreme outlier rates, \name produces slightly lower estimation errors compared to ground truth, further validating that the results of GORE can be suboptimal. 

%%%%%%%%%%%%%%%%%%%%%%%%%
\input{fig-benchmark_extreme_outlier}
%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{\name in Robotics}
\label{sec:roboticsApplication}
\todo.


%\grayout{
%from [0]: The source code for the compared methods were released by the authors. Go-ICP and Glob-GM-ML are implemented in C++, while APM is implemented using MATLAB. Our algorithms are all implemented in C. All the experiments were conducted on a computer equipped with an Intel Xeon E5 3.2 GHz CPU.
%
%
%[0] downsamples typical registration benchmarks (typically >10k points) to contain ~500 points
%
%Performance metrics:
%\bit
%\item runtime: of each stage
%\item rotation error
%\item translation error (with and without refinement?)
%\item RMS error between point clouds (with gt correspondences) produced by each approach
%\eit
%terminate slow approaches after 1000s
%
%Experimental setup in [0]:
%\bit
%\item get 500 points
%\item add different ratios of outliers
%\item  apply random transformation
%\item add some noise 
%\eit
%}

==> sections/old/old-example-TLSMaxConsensus.tex <==
%!TEX root = ../main.tex

\begin{example}[\TLS vs. Consensus Maximization]
Consider a simple scalar estimation problem, where we are given three measurements $s_1\!=\!s_2\!=\!0$ %$k=1,\ldots,K-1$ 
and $s_3 = 3$. Assume $\alpha_k = 2$, $k=1,2,3$ and $\barc=1$. 
Then, it is possible to see that $s_{m} = 1.5$ attains a maximum consensus set including all measurements $\{1,2,3\}$, while the \TLS estimate is $\hats = 0$ which attains a cost $f_s(\hats) = 1$, and has consensus set $\calC(\hats) = \{1,2\}$.
\end{example}

%!TEX root = main.tex

\section{Comments on TLS vs. Consensus Maximization}
\label{sec:exampleTLSMaxConsensus}

\TLS (and Algorithm~\ref{alg:adaptiveVoting}) are related to \emph{consensus maximization}, a popular approach for outlier detection in vision~\cite{Speciale17cvpr-consensusMaximization,Liu18eccv-registration}. 
Consensus maximization looks for an estimate that maximizes the number of inliers, i.e. $\max_s |\calC(s)|$, where $|\cdot|$ denotes the cardinality of a set.
While consensus maximization is intractable in general, by following the same lines of Theorem~\ref{thm:scalarTLS}, it is easy to show that consensus maximization can be solved in polynomial time in the scalar case as $\argmax_{i,\ldots,2K-1} |\calC_i|$. While we expect the \TLS solution to maximize the set of inliers, consensus maximization and \TLS will not return the same solution in general, since \TLS may prefer to discard measurements that induce a large bias in the estimate, as shown by the simple example below.

\begin{example}[\TLS vs. Consensus Maximization]
Consider a simple scalar estimation problem, where we are given three measurements $s_1\!=\!s_2\!=\!0$ %$k=1,\ldots,K-1$ 
and $s_3 = 3$. Assume $\alpha_k = 2$, $k=1,2,3$ and $\barc=1$. 
Then, it is possible to see that $s_{m} = 1.5$ attains a maximum consensus set including all measurements $\{1,2,3\}$, while the \TLS estimate is $\hats = 0$ which attains a cost $f_s(\hats) = 1$, and has consensus set $\calC(\hats) = \{1,2\}$.
\end{example}

==> sections/old/old-robustRegistrationSubproblems.tex <==
%!TEX root = ../main.tex

\section{Solving the Registration Subproblems}
\label{sec:subproblems}

% The following sections describe how to obtain global and robust estimates of scale (Section~\ref{sec:scaleEstimation}),
% rotation (Section~\ref{sec:rotationEstimation}), and translation (Section~\ref{sec:translationEstimation}). 

==> sections/old/old-scaleEstimation.tex <==
%!TEX root = ../main.tex

\subsection{Robust Scale Estimation}
\label{sec:scaleEstimation}

% In this section we use the translation and rotation invariant measurements in eq.~\eqref{eq:TRIM} to 
% estimate the scale $s$. 
The generative model~\eqref{eq:TRIM} describes linear measurements $s_{ij}$ of the unknown scale $s$, affected 
by bounded noise $|\eps^s_{ij}| \leq \alpha_{ij}$ including potential outliers (when $o^s_{ij} \neq 0$).
Again, we estimate the scale given the measurements $s_{ij}$ and the bounds $\alpha_{ij}$ using a 
\TLS estimator:

\vspace{-5mm}
\bea
\label{eq:TLSscale}
\hats = \argmin_{s} \sumAllIM \min\left( \frac{  (  s-s_k )^2 }{  \alpha^2_k }  \;,\; \barcsq \right)
\eea
where for simplicity we numbered the measurements from $1$ to $K = |\calE|$ and adopted the notation $s_k$ instead of $s_{ij}$.
% From the previous section we have a bunch of measurements of the scale, potentially affected by outliers:
% \bea
% s_k \doteq \frac{  \|  \vb_{ij} \| }{  \|  \va_{ij} \| }  = s + \hat{o}_{ij} 
% \eea
% \TLS estimator:
% %
% \bea
% \label{eq:TLSscale}
% % s^\star = \argmin_{s} \sumAllPoints \min\left( (s - s_k)^2 , \barcsq \right)
% s^\star = \argmin_{s,\theta_k \in \{-1,+1\}} 
% \sumAllPoints \frac{(1+\theta_k)}{2}  \frac{(s - s_k)^2}{\sigma_s^2}  + \frac{(1-\theta_k)}{2}  \barcsq 
% \eea

The following theorem shows that one can solve~\eqref{eq:TLSscale} in polynomial time by a simple enumeration. 

\begin{theorem}[Optimal \TLS Scale Estimation]\label{thm:scalarTLS}
For a given $s \in \Real{}$, define the \emph{consensus set of $s$} as $\calC(s) = \setdef{k}{ \frac{  (  s-s_k )^2 }{  \alpha^2_k } \leq \barcsq }$. 
Then, for any $s \in \Real{}$, there are at most $2\nrTIM-1$ different non-empty consensus sets. If we name these sets $\calC_1, \ldots, \calC_{2K-1}$, then the solution of~\eqref{eq:TLSscale} can be computed by enumeration as:
\bea
\hats = \argmin 
\left\{ 
f_s(\hats_i) : \hats_i = 
\left(\sum_{k\in\calC_i} \frac{1}{\alpha_k^2} \right) \inv \sum_{k\in\calC_i} \frac{s_k}{\alpha_k^2}, \forall i 
\right\}
\eea   
where $f_s(\cdot)$ is the objective function of~\eqref{eq:TLSscale}. 
\end{theorem}
% consensus maximization is a popular framework~\cite{Speciale17cvpr-consensusMaximization,Liu18eccv-registration}, 
% A proof of~\prettyref{thm:scalarTLS} is  given in Appendix~\ref{sec:proof:scalarTLS}.

\prettyref{thm:scalarTLS}, whose proof is given in the \supp, is based on the insight 
that the consensus set can only change at the boundaries of the intervals $[s_k - \alpha_k\barc, s_k + \alpha_k\barc]$ (Fig.~\ref{fig:consensusMax}(a)) and there are at most $2\nrTIM$ such boundaries. The theorem
also suggests a straightforward \emph{adaptive voting} algorithm to solve~\eqref{eq:TLSscale}, with pseudocode given in Algorithm~\ref{alg:adaptiveVoting}. The algorithm first builds the boundaries of the 
intervals shown in Fig.~\ref{fig:consensusMax}(a) (line~\ref{line:boundaries}). Then, for each interval, it evaluates the consensus set (line~\ref{line:consensusSet}, see also Fig.~\ref{fig:consensusMax}(b)). 
Since the consensus set does not change within an interval, we compute it at the interval centers (line~\ref{line:midPoints}, see also Fig.~\ref{fig:consensusMax}(b)). Finally, the cost of each consensus set is computed and the smallest cost is returned as optimal solution (line~\ref{line:enumeration}).  
% First, if we attach a confidence interval $[s_k - \alpha_k\barc, s_k + \alpha_k\barc]$ 
% to each measurement $s_k$, then every $s$ in the $k$-th interval satisfies $\frac{\|s-s_k\|^2}{\alpha_k^2} \leq \barcsq$ and 
% $k$ is in the consensus set of $s$ (Fig.~\ref{fig:consensusMax}(a)). %is in the consensus set of $k$.
% As a consequence, the consensus set can only change at the boundary of the intervals $[s_k - \alpha_k\barc, s_k + \alpha_k\barc]$ and there are at most $2\nrTIM-1$ such intervals (Fig.~\ref{fig:consensusMax}(b)).
% Second, problem~\eqref{eq:TLSscale} simply computes the least squares estimate of the measurements in the consensus set of the solution. Therefore, we can just enumerate every possible consensus set and compute a least squares estimate for each of them,
% to find the solution that induces the smallest cost. 
% The one leading to the smaller cost is then 
% Problem~\eqref{eq:TLSscale} computes the \TLS estimate of a set of scalars $s_k$, each one associated with a bound $\alpha_k$. In particular, for any $s$ the cost~\eqref{eq:TLSscale} computes the least squares deviation of the measurements in the consensus set $\calC_i$ and then add $\barcsq$ for each of the remaining measurements. The problem can be visualized as in Fig.~\ref{fig:consensusMax}(a): where we see the measured scalars $s_1, s_2, \ldots$ and the corresponding intervals $[s_k-\alpha_k, s_k+\alpha_k]$. Then a measurement $k$ is in the consensus set of $s$ if the $s$ belongs to the interval $[s_k-\alpha_k, s_k+\alpha_k]$. From the figure it is clear that a consensus set can only change when crossing the boundaries $[s_k-\alpha_k, s_k+\alpha_k]$ (shown in red) for some $k$. Since there are $K$ measurements, we have at most $2K$ boundaries, which define $2K-1$ intervals, proving the first part of the theorem. 
% The second part trivially follows from the fact that the consensus set of $\hats$ is necessarily one of the $2K-1$ possible consensus sets.  


% ========================
\input{./sections/fig-adaptiveVoting} 
% ========================

% ========================
\input{./sections/algo-adaptiveVoting}
% \vspace{-15mm}
% ========================
% estimate must be positive: convex combination of positive quantities


The interested reader can find a discussion on the relation between \TLS and \emph{consensus maximization} (a popular approach for outlier detection~\cite{Speciale17cvpr-consensusMaximization,Liu18eccv-registration}) in the \supp.
% are encouraged to refer to the \supp\ for comments on \TLS (and Algorithm~\ref{alg:adaptiveVoting}) and \emph{consensus maximization}, a popular approach for outlier detection in vision~\cite{Speciale17cvpr-consensusMaximization,Liu18eccv-registration}.

% We conclude this section by noting that \TLS (and Algorithm~\ref{alg:adaptiveVoting}) are related to \emph{consensus maximization}, a popular approach for outlier detection in vision~\cite{Speciale17cvpr-consensusMaximization,Liu18eccv-registration}. 
% Consensus maximization looks for an estimate that maximizes the number of inliers, i.e. $\max_s |\calC(s)|$, where $|\cdot|$ denotes the cardinality of a set.
% While consensus maximization is intractable in general, by following the same lines of Theorem~\ref{thm:scalarTLS}, it is easy to show that consensus maximization can be solved in polynomial time in the scalar case as $\argmax_{i,\ldots,2K-1} |\calC_i|$. While we expect the \TLS solution to maximize the set of inliers, consensus maximization and \TLS will not return the same solution in general, since \TLS may prefer to discard measurements that induce a large bias in the estimate, as shown by an example in the \supp.
%pointed out in the following example.
% moved to supplementary
% \begin{example}[\TLS vs. Consensus Maximization]
% Consider a simple scalar estimation problem, where we are given three measurements $s_1\!=\!s_2\!=\!0$ %$k=1,\ldots,K-1$ 
% and $s_3 = 3$. Assume $\alpha_k = 2$, $k=1,2,3$ and $\barc=1$. 
% Then, it is possible to see that $s_{m} = 1.5$ attains a maximum consensus set including all measurements $\{1,2,3\}$, while the \TLS estimate is $\hats = 0$ which attains a cost $f_s(\hats) = 1$, and has consensus set $\calC(\hats) = \{1,2\}$.
% \end{example}
% 
% \myParagraph{Example (\TLS vs. Consensus Maximization)}   
% \vspace{1cm}
% \bea
% s_1 \quad 
% s_1 - \alpha_1 \quad
% s_1 + \alpha_1 \quad \\
% s_1 \quad s_2 \quad s_3 \quad s_4 \quad s_5 \\
% \alpha_1 \quad \alpha_2 \quad \alpha_3 \quad \alpha_4 \quad \alpha_5 
% \eea



{\bf What if the scale is known?} 
In some registration problems, the scale is known, e.g., the scale of the two point clouds is the same. In such a case, we can skip Algorithm~\ref{alg:adaptiveVoting} and set $\hats$ to be the known scale. 
Moreover, we can still use the \mcis method to largely reduce the number of outliers.
% Moreover, we introduce an outlier rejection method based on graph theory. For all the TRIMs $\{s_{ij} \}$ generated from Eq.~\eqref{eq:TRIM}, we can discard those TRIMs such that $\frac{|s_{ij} - \hats|}{\alpha_{ij}^2} > \barcsq=1$, which is equal to removing the edge $\{i,j\}$ in the edge set of the original fully connected graph $\calG=\{\calV,\calE\}$. 



==> sections/old/relatedWork-old.tex <==
%!TEX root = ../main.tex

\section{Related Work}
\label{sec:relatedWork}
There are two established paradigms for the registration of 3D point clouds: 
\emph{Correspondence-based} and 
\emph{Simultaneous Pose and Correspondence} methods. 
% alternate between finding the correspondences and computing the best transformation.
%%%%%%
% There are two established paradigms for the registration of 3D point clouds: 
% \emph{correspondence-based} methods extract and match 3D keypoints in the point clouds and 
% then solve for the optimal transformation, while 
% \emph{Simultaneous Pose and Correspondence} (\SPC) methods 
% alternate between finding the correspondences and computing the best transformation.
%%%%%
% one that iteratively alternates between finding the correspondences and computing the best transformation, also known as \emph{simultaneous pose and correspondence} (SPC) paradigm, and the other that first computes the correspondences using keypoint matching methods and then solve the optimal transformation, and we review them separately.

% ==================================================================================
\subsection{Correspondence-based Methods}
Correspondence-based methods first detect and match 3D keypoints between point clouds using local~\cite{Tombari13ijcv-3DkeypointEvaluation,Guo14pami-3Dkeypoints,Rusu08iros-3Dkeypoints,Rusu09icra-fast3Dkeypoints} or global~\cite{Drost10cvpr,Koppula11nips} descriptors to establish putative correspondences, and then either use closed-form solutions~\cite{Horn87josa,Arun87pami} in a \ransac~\cite{Fischler81} scheme, or apply robust optimization methods~\cite{Zhou16eccv-fastGlobalRegistration,Bustos18pami-GORE} to gain robustness against outliers. 3D keypoint matching is 
known to be less accurate compared to 2D counterparts like \SIFT and \ORB,
% \SIFT~\cite{lowe2004ijcv-distinctive} and \ORB~\cite{rublee2011iccv-orb},
% due to essential complexity and lack of distinctive features in point clouds, 
thus causing much higher outlier rates, e.g., having 95\% spurious correspondences is considered common~\cite{Bustos18pami-GORE}. Therefore, a robust backend that can deal with extreme outlier rates is highly desirable.
% urgently required for accurate pose estimation. 

\myParagraph{Registration without outliers} Horn~\cite{Horn87josa} and Arun~\cite{Arun87pami} show that optimal solutions 
(in the maximum likelihood sense) for scale, rotation, and translation can be computed in closed form 
when the points are affected by isotropic zero-mean Gaussian noise.
%, and assuming
%in the least squares sense under Gaussian noise distribution 
 % all the correspondences are known and correct. 
 Olsson\setal~\cite{olsson2009pami-branch} propose a method based on \bnb that is globally optimal and allows point-to-point, point-to-line, and point-to-plane correspondences. Recently, Briales and Gonzalez-Jimenez~\cite{Briales17cvpr-registration} propose a semidefinite relaxation that can deal with anisotropic Gaussian noise, and has per-instance optimality guarantees. 
 % However, these methods are known to perform badly at the presence of even a single outlier.
 % All these methods assume that all the correspondences are known and correct.

\myParagraph{Robust registration} Probably the most widely used robust registration approach is based on \ransac~\cite{Fischler81,Chen99pami-ransac}, which has enabled several early applications in vision and robotics~\cite{Hartley00,Meer91ijcv-robustVision}. Despite its efficiency in the low-noise and low-outlier regime, \ransac exhibits slow convergence and low accuracy 
 with large outlier rates~\cite{Bustos18pami-GORE}, where it becomes harder to sample a ``good'' consensus set.
 % with large noise and high outlier rates and it loses optimality guarantee because not all the inliers can be kept at convergence. 
 Other approaches resort to \emph{M-estimation}, which replaces the least squares objective function with robust costs that are less sensitive to outliers~\cite{MacTavish15crv-robustEstimation,Black96ijcv-unification,Lajoie19ral-DCGM}. Zhou\setal~\cite{Zhou16eccv-fastGlobalRegistration} propose \emph{Fast Global Registration} (\FGR) that uses the Geman-McClure cost function and leverages 
 % the Black-Rangarajan duality and  
 graduated non-convexity to solve the resulting non-convex optimization.
 % through multiple iterations of Horn's method~\cite{Zhou16eccv-fastGlobalRegistration}. 
 Since graduated non-convexity has to be solved in discrete steps, \edit{\FGR} does not guarantee global optimality~\cite{Bustos18pami-GORE}. Indeed, \FGR tends to fail when the outlier ratio is high (>80\%), as we show in~\prettyref{sec:experiments}.
 % is only robust to modest level of outliers (e.g. 10\%-70\%), and tends to fail when the outlier ratio is extremely high (>80\%), which will be shown in \prettyref{sec:experiments}. 
 Bustos and Chin~\cite{Bustos18pami-GORE} propose a \emph{Guaranteed Outlier REmoval} (\GORE) technique, that uses 
 % In addition,  has been recently demonstrated by  to use 
 geometric operations to significantly reduce the amount of outlier correspondences before passing them to the optimization backend. \GORE has been shown to be robust to 95\% spurious correspondences~\cite{Bustos18pami-GORE}. 
 However, \GORE does not estimate the \emph{scale} of the registration and has exponential worst-case time complexity due to the possible usage of \bnb (see Algorithm 2 in~\cite{Bustos18pami-GORE}).

 \LC{Quasar is first polynomial-time certifiably robust algorithm. but slow..}

 \LC{TEASER is ultra-robust and polynomial-time but slow, and unclear end-to-end guarantees.}
 % \GORE can be considered a pre-processing step, rather than a registration technique. More importantly, 
 % it does not provide means to estimate the \emph{scale} of the registration.\todo{more on BnB?}
  % resulting in robustness to >95\% outlier ratios~\cite{Bustos18pami-GORE}. Nevertheless, GORE itself only focuses on outlier pruning and does not output accurate transformation. Furthermore, the outlier rejection scheme in GORE is complex, hard to interpret, and takes considerable computation. Instead, as shown in \prettyref{sec:scaleEstimation}, after scale estimation, our algorithm uses straightforward scale invariance and graph theory to significantly reject outliers and decrease the problem size, which has similar robustness to extremely high outlier rates.
% \myParagraph{Novelty} 
% polynomial time
% general

% ==================================================================================
\subsection{Simultaneous Pose and Correspondence Methods}
\emph{Simultaneous Pose and Correspondence} (\SPC) methods 
 alternate between finding the correspondences and computing the best transformation given the correspondences.

\myParagraph{Local methods} The \emph{Iterative Closest Point} (\ICP) algorithm~\cite{Besl92pami} is considered a milestone in point cloud registration. 
% and remains one of the most widely used approaches. 
However, \ICP is \edit{prone to converge}
% known for its vulnerability 
 to \emph{local minima} and it only performs well given a good initial guess. 
% of the transformation.
%without good initial guesses, due to the high nonconvexity of the problem. 
Multiple variants of \ICP~\cite{Granger02eccv,Sandhu10pami-PFregistration,Zhang16sp-robustICP,
Maier12pami-convergentICP,Chetverikov05ivc-trimmedICP,Kaneko03pr-robustICP,
Bouaziz13acmsig-sparseICP} \edit{have proposed to use}
 % showing that the use of 
 robust cost functions to improve convergence.
 % and better convergence has been observed with robust kernels. 
Probabilistic interpretations have also been proposed to improve \ICP convergence, for instance interpreting the registration problem as a minimization of the Kullback-Leibler divergence between two Gaussian Mixture Models~\cite{Jian05iccv-registrationGMM,Myronenko10pami-coherentPointDrift,Jian11pami-registrationGMM,Campbell15iccv-adaptiveRegistration}. 
All these methods rely on iterative local search, do not provide global optimality guarantees, and typically fail 
without a good initial guess.
% no global optimality can be guaranteed.

\myParagraph{Global methods} Global \SPC approaches compute a globally optimal solution without initial guesses,
% register point clouds to guaranteed global optima without requirement of an initial guess 
and are usually based on \bnb, which at each iteration divides the parameter space into multiple sub-domains (branch) and computes the bounds of the objective function for each sub-domain (bound). A series of geometric techniques have been proposed to improve the bounding tightness~\cite{Hartley09ijcv-globalRotationRegistration,
Breuel03cviu-BnBimplementation,Yang16pami-goicp,
Campbell16cvpr-gogma,Parra14cvpr-fastRotationRegistration} and increase the search speed~\cite{Yang16pami-goicp,Li19arxiv-fastRegistration}. However, the runtime of \bnb increases exponentially with the size of the point cloud and it can be made worse by the explosion of the number of local minima resulting from high outlier ratios~\cite{Bustos18pami-GORE}. \edit{Global SPC registration can  be also formulated as a mixed-integer program~\cite{Izatt17isrr-MIPregistration}, though the runtime remains exponential.}

\LC{add this: \url{https://ieeexplore.ieee.org/abstract/document/8870243}}
\LC{add this: \url{https://arxiv.org/abs/1908.02021}}
% \myParagraph{Correspondence-based vs. \SPC} %While the \SPC 
% It is worth noting that 
% an \SPC problem can be reformulated as a correspondence-based problem by adding point correspondences 
% between any pair of points in the two cloud. This is typically imp


\myParagraph{Deep learning methods} \LC{add here}.. but no guarantees. 
in experiments we do better, etc.

\subsection{Wahba problem without outliers}
The Wahba problem was first proposed by Grace Wahba in 1965 with the goal of estimating satellite attitude given vector observations~\cite{wahba1965siam-wahbaProblem}. 
In aerospace, the vector observations are typically the directions to visible stars observed by sensors onboard the satellite.
The Wahba problem~\eqref{eq:wahbaProblem} is related to the well-known 
%an alternative formulation of the well-known 
\emph{Orthogonal Procrustes} problem~\cite{Gower05oss-procrustes} where one searches for 
orthogonal matrices (rather than rotations) and all the weights $w_i$ are set to be equal to one.
Schonemann~\cite{Schonemann66psycho} provides a closed-form solution for the Orthogonal Procrustes problem using
 singular value decomposition. 
% The Orthogonal Procrustes problem can be solved in closed form using
%  singular value decomposition~\cite{Schonemann66psycho}. 
 Subsequent research effort across multiple communities led to the derivation of 
 %Later, researchers from different communities have derived 
 closed-form solutions for the Wahba problem~\eqref{eq:wahbaProblem} using both quaternion~\cite{Horn87josa,markley2014book-fundamentalsAttitudeDetermine} and rotation matrix~\cite{horn1988josa-rotmatsol,markley1988jas-svdAttitudeDeter,Arun87pami,Forbes15jgcd-wahba,Saunderson15siam,Khoshelham16jprs} representations. 

The computer vision community has investigated the Wahba problem in the context of  
 point cloud registration~\cite{Besl92pami,Yang16pami-goicp}, image stitching~\cite{Bazin14eccv-robustRelRot}, motion estimation and 3D reconstruction~\cite{Blais95pami-registration,Choi15cvpr-robustReconstruction}. 
 In particular, the closed-form solutions from  
 Horn~\cite{Horn87josa} and Arun\setal~\cite{Arun87pami} 
 are now commonly used in point cloud registration techniques~\cite{Besl92pami}. 
 While the formulation~\eqref{eq:wahbaProblem} implicitly assumes zero-mean isotropic Gaussian noise, 
 several authors investigate a generalized version of the Wahba problem~\eqref{eq:wahbaProblem}, where the noise follows an anisotropic Gaussian~\cite{Briales17cvpr-registration,cheng2019aiaaScitech-totalLeastSquares,Crassidis07-survey}. 
 % Recent effort includes the development of solvers for the anisotropic case. 
 Cheng and Crassidis~\cite{cheng2019aiaaScitech-totalLeastSquares} develop a local iterative optimization algorithm. Briales and Gonzalez-Jimenez~\cite{Briales17cvpr-registration} propose a convex relaxation to compute global solutions for the anisotropic case. 
 Ahmed\setal~\cite{Ahmed12tsp-wahba} develop an SDP relaxation for the case with bounded noise and no outliers.
  % and we refer the reader to~\cite{markley2014book-fundamentalsAttitudeDetermine} for a comprehensive review.  On the other hand,
 % , with the underlying assumption of zero-mean isotropic Gaussian noise distribution. Recently, although in solving a different problem, Briales and Gonzalez-Jimenez propose a convex semidefinite relaxation that can handle large anisotropic Gaussian no{}ise in point cloud registration with per-instance optimality guarantees~\cite{Briales17cvpr-registration}. 
 All these methods %assume the measurement noise to be Gaussian (in other words: no wrong correspondences), and 
 are known to perform poorly in the presence of outliers.
% Typical examples are the unit vectors giving the direction to the sun or a star and the unit vector in the
% direction of the Earth’s magnetic field.

\subsection{Wahba problem with outliers} 

In computer vision applications, the vector-to-vector correspondences are typically established through descriptor matching, which may lead to spurious correspondences and outliers~\cite{Bustos2015iccv-gore3D,Bustos18pami-GORE}. This observation triggered research into outlier-robust variants of the Wahba problem.
%, that can tolerate outliers.

\myParagraph{Local Methods} The most widely used method for handling outliers is \ransac, which is efficient and accurate in the low-noise and low-outlier regime~\cite{Fischler81,Meer91ijcv-robustVision}. However, \ransac is non-deterministic (different runs give different solutions), sub-optimal (the solution may not capture all the inlier measurements), and its performance quickly deteriorates in the large-noise and high-outlier regime. Other approaches resort to \emph{M-estimators}, which replace the least squares cost in eq.~\eqref{eq:wahbaProblem} with robust cost functions that are less sensitive to outliers~\cite{Black96ijcv-unification,MacTavish15crv-robustEstimation}. Zhou \etal~\cite{Zhou16eccv-fastGlobalRegistration} propose \emph{Fast Global Registration} (\FGR) that employs the Geman-McClure robust cost function and solves the resulting optimization iteratively using a continuation method. 
%via graduated non-convexi
% by gradually increasing the non-convexity. 
Since the problem becomes more and more non-convex at each iteration, \FGR does not guarantee global optimality in general. In fact, as we show in Section \ref{sec:experiments}, \FGR tends to fail when the outlier ratio is above 70\% of the observations. 

\myParagraph{Global Methods} The most popular class of global methods for robust rotation search is based on \emph{Consensus Maximization}~\cite{chin2017slcv-maximumconsensusadvances} and \emph{branch-and-bound} (\bnb)~\cite{campbell2017iccv-2D3Dposeestimation}. Hartley and Kahl~\cite{Hartley09ijcv-globalRotationRegistration} first proposed using \bnb for rotation search, and Bazin \etal~\cite{bazin2012accv-globalRotSearch} adopted consensus maximization to extend their \bnb algorithm with a robust formulation. \bnb is guaranteed to return the globally optimal solution, but it runs in exponential time in the worst case. % due to exhaustive search space exploration. 
Another class of global methods for consensus maximization enumerates all possible subsets of measurements with size no larger than the problem dimension (3 for rotation search) to analytically compute candidate solutions, and then verify global optimality using computational geometry~\cite{olsson2008cvpr-polyRegOutlier,enqvist2012eccv-robustfitting}. These methods 
still require exhaustive enumeration.  
% exhibit exhaustive enumeration and typically require iterative local optimization and global verification.
% leverages the fact that the solution to the original problem on all data points is equivalent to the same problem on a subset of at most $d$ points, where $d=3$ for rotation search~\cite{olsson2008cvpr-polyRegOutlier,enqvist2012eccv-robustfitting}. Such methods thus enumerate all possible $\left( \substack{N \\ p} \right)$ subsets of measurements with $p\leq d$ to 
% %analytically 
% compute the rotation. These methods, however, still require exhaustive enumeration.
% Despite exhaustive enumeration, these techniques demonstrate successful performance on similar applications.  

\myParagraph{Outlier-removal Methods} Recently, Para and Chin~\cite{Bustos2015iccv-gore3D} proposed a \emph{guaranteed outlier removal} (\GORE) algorithm that removes gross outliers while ensuring that all inliers are preserved. %, even in the presence of extreme amount of outliers. 
Using \GORE as a preprocessing step for \bnb is shown to boost the speed of \bnb, while using \GORE alone still provides a reasonable sub-optimal solution. Besides rotation search, \GORE has also been successfully applied to other geometric vision problems such as triangulation~\cite{Chin16cvpr-outlierRejection}, and registration~\cite{Bustos2015iccv-gore3D,Bustos18pami-GORE}. Nevertheless, 
 the existing literature is still missing a polynomial-time algorithm that can
% an algorithm that can 
simultaneously tolerate extreme amounts of outliers and return globally optimal solutions.
% is still highly desired. 

%\grayout{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Robust Statistics}
%
%based on high-level overview [Robust Statistics for outlier detection].
%\bit
%\item univariate: median, M-estimators, scoring methods
%\item multivariate: min covariance determinant (combinatorial search), M-estimators,
%least trimmed squares
%\eit
%
%Important aspects:
%\bit
%\item efficiency
%\item breakdown point
%\item influence function
%\eit
%
%differences:
%\bit
%\item we consider nonconvex setup, and don't try to recover covariances
%\item we may have bounds instead Least Trimmed Squares (LTS) assume fixed fraction of inliers
%\item 
%\eit
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Robust Regression in Computer Vision and Robotics}
%mainly pointers to surveys:
%\bit
%\item Robust regression methods for computer vision: A review: \url{https://link.springer.com/article/10.1007/BF00127126}
%\item SLAM: 
%\eit
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Robust Registration (Pose Estimation)}
%
%from [0]: Fast and Globally Optimal Rigid Registration of
%3D Point Sets by Transformation Decomposition.
%Add also: Efficient Global Point Cloud Registration by
%Matching Rotation Invariant Features Through
%Translation Search~\cite{Liu18eccv-registration} (conference version of [0]) \todo: understand carefully the differences
%\bit
%\item closed forms without outliers:
%	\bit
%	\item point to point, isotropic: Horn, Arun
%	\item general: Briales
%	\eit
%\item approaches with outliers:
%	\bit
%	\item RANSAC [9]-[12] in [0]
%	\eit
%\item approaches without correspondences (SPC = Simultaneous Pose and Correspondence)
%	\bit
%	\item ICP and variants: [15]-[24] in [0]
%	\item alignment of distributions: [25]-[31] in [0]
%	\item BnB: [32]-[39] in [0]
%		\bit
%		\item using l2 norm [32]
%		\item consensus set maximization: using consensus points with l2 norm [38]-[39]
%		\item consensus set maximization: using consensus points with linf norm [0]. Decouple translation and rotation and use a clever data structure (3D integral volumes) to speed up computation. 
%		Issues of [0]:
%			\bit
%			\item a lot of random pre=processing of points
%			\item very small noise (0.01?)
%			\eit
%		\eit
%	\eit
%\eit
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Robust Rotation Estimation}
%[38]-[49] in [0]
%}

==> sections/proof-prop-naiveRelax.tex <==
%!TEX root = main.tex

\section{Proof of Proposition~\ref{prop:naiveRelax}}
\label{sec:proof:prop:naiveRelax}
\begin{proof}
We show eq.~\eqref{eq:naiveRelaxation} is a convex relaxation of~\eqref{eq:qcqpZ} by showing that (i) eq.~\eqref{eq:naiveRelaxation} is a relaxation (\ie, the constraint set of~\eqref{eq:naiveRelaxation} includes the one of~\eqref{eq:qcqpZ}), and (ii) eq.~\eqref{eq:naiveRelaxation} is convex. (i) is true because from~\eqref{eq:qcqpZ} to~\eqref{eq:naiveRelaxation} we have dropped the $\rank{\MZ}=1$ constraint. Therefore, the feasible set of~\eqref{eq:qcqpZ} is a subset of the feasible set of~\eqref{eq:naiveRelaxation}, and the optimal cost of~\eqref{eq:naiveRelaxation} is always smaller or equal than the optimal cost of~\eqref{eq:qcqpZ}. To prove (ii), we note that the objective function and the constraints of~\eqref{eq:naiveRelaxation} are all linear in $\MZ$, and $\MZ\succeq 0$ is a convex constraint, hence~\eqref{eq:naiveRelaxation} is a convex program.
\end{proof}

==> sections/proof-prop-relaxationRedundant.tex <==
%!TEX root = main.tex

\section{Proof of Proposition~\ref{prop:relaxationRedundant}}
\label{sec:proof:prop:relaxationRedundant}
\begin{proof}
Here we prove that eq.~\eqref{eq:relaxationRedundant} is a convex relaxation of eq.~\eqref{eq:qcqpZ}
and that the relaxation is always tighter, \ie the optimal objective  of~\eqref{eq:SDPrelax} is always closer to the optimal objective of~\eqref{eq:TLSBinaryClone}, when compared to the naive relaxation~\eqref{eq:naiveRelaxation}.

To prove the first claim, we first show that the additional constraints in the last two lines of~\eqref{eq:SDPrelax} are 
\emph{redundant} for~\eqref{eq:qcqpZ}, \ie, they are trivially satisfied by any feasible solution of~\eqref{eq:qcqpZ}.
Towards this goal  
% , we show that (i)~\eqref{eq:relaxationRedundant} is convex and (ii)~\eqref{eq:relaxationRedundant} is a relaxation. 
%
% (i) is easy to show because the objective function and all the constraints in~\eqref{eq:relaxationRedundant} are linear in $\MZ$ (and $\MZ\succeq 0$ is a convex set), and therefore the SDP is convex. To show (ii), 
we note that eq.~\eqref{eq:qcqpZ} is equivalent to~\eqref{eq:TLSBinaryClone}, where $\vxx$ is a column vector stacking $N+1$ quaternions: $\vxx = [\vq\tran\ \vq_1\tran\ \dots \vq_N\tran]\tran$, and where each $\vq_i = \theta_i \vq,\theta_i \in \{\pm 1\},\forall i=1,\dots,N$. Therefore, we have:
\bea
{[\MZ]_{qq_i} = \vq \vq_i\tran = \theta_i\vq \vq\tran = \vq_i \vq\tran = (\vq \vq_i\tran)\tran = [\MZ]\tran_{qq_i} } 
\nonumber \\
{ [\MZ]_{q_iq_j} = \vq_i \vq_j\tran = \theta_i\theta_j\vq \vq\tran = \vq_j \vq_i\tran = (\vq_i \vq_j\tran)\tran = [\MZ]\tran_{q_iq_j} }
\nonumber %\\
\eea
This proves that the constraints $[\MZ]_{qq_i} = [\MZ]\tran_{qq_i}$ and $[\MZ]_{q_iq_j} = [\MZ]\tran_{q_iq_j}$ are redundant for~\eqref{eq:qcqpZ}.
% , i.e., they are trivially satisfied by any feasible solution of~\eqref{eq:qcqpZ}. 
Therefore, problem~\eqref{eq:qcqpZ} is equivalent to:
\bea 
\label{eq:qcqpZredundant}
\min_{\MZ \succeq 0} & \trace{\MQ \MZ} \\
\subject %& \MZ \succeq 0 \nonumber \\
& \trace{[\MZ]_{qq}} = 1 \nonumber \\
& [\MZ]_{q_i q_i} = [\MZ]_{qq}, \forall i=1,\dots,N \nonumber \\
& [\MZ]_{q q_i} = [\MZ]\tran_{q q_i}, \forall i=1,\dots,N \nonumber \\
& [\MZ]_{q_i q_j} = [\MZ]\tran_{q_i q_j}, \forall 1\leq i < j \leq N \nonumber \\
& \rank{\MZ} = 1 \nonumber
\eea 
where we added the redundant constraints as they do not alter the feasible set.
At this point, proving that~\eqref{eq:relaxationRedundant} is a convex relaxation of~\eqref{eq:qcqpZredundant} 
(and hence of~\eqref{eq:qcqpZ}) can be done with the same arguments of the proof of Proposition~\ref{prop:naiveRelax}:  
in~\eqref{eq:relaxationRedundant} we dropped the rank constraint (leading to a larger feasible set) and the remaining constraints 
are convex.


 % the feasible set of eq.~\eqref{eq:relaxationRedundant} cannot be smaller than the feasible set of eq.~\eqref{eq:qcqpZ}, which means~\eqref{eq:relaxationRedundant} is still a relaxation of~\eqref{eq:qcqpZ}. 
The proof of the second claim is straightforward.
 Since we added more constraints in~\eqref{eq:relaxationRedundant} compared to the naive relaxation~\eqref{eq:naiveRelaxation}, the optimal cost of~\eqref{eq:relaxationRedundant} always achieves a higher objective than~\eqref{eq:naiveRelaxation}, 
and since they are both relaxations, their objectives provide a lower bound 
  to the original non-convex problem~\eqref{eq:qcqpZ}.
\end{proof}

==> sections/proof-theorem-strongDuality.tex <==
%!TEX root = main.tex

\section{Proof of Theorem~\ref{thm:strongDualityNoiseless}}
\label{sec:proof:theorem:strongDuality}
\begin{proof}
To prove Theorem~\ref{thm:strongDualityNoiseless}, we first use Lagrangian duality to derive the \emph{dual} problem of the \QCQP in~\eqref{eq:TLSBinaryClone}, and draw connections to the naive SDP relaxation in~\eqref{eq:naiveRelaxation} (Section~\ref{sec:LagrangianandWeakDuality}). 
%
Then we leverage the well-known \emph{Karush-Kuhn-Tucker} (KKT) conditions~\cite{Boyd04book} to prove a general sufficient condition for tightness, as shown in Theorem~\ref{thm:generalStrongDuality} (Section~\ref{sec:KKTStrongDuality}). 
%As we will see, \emph{tightness} of the relaxation~\eqref{eq:naiveRelaxation} is equivalent to \emph{}
%
Finally, in Section~\ref{sec:strongDualityNoiselessOutlierfree}, we demonstrate that in the case of no noise and no outliers, we can provide a constructive proof to show the sufficient condition in Theorem~\ref{thm:generalStrongDuality} always holds.


\subsection{Lagrangian Function and Weak Duality}
\label{sec:LagrangianandWeakDuality}
Recall the expressions of $\MQ_i$ in eq.~\eqref{eq:Qi}, and define $\MQ = \sumAllPointsi \MQ_i$.
The matrix $\MQ$ has the following block structure:
\bea
\hspace{-5mm}
& \MQ = \sumAllPointsi \MQ_i 
% \\& 
= 
\bmat{c|ccc}
\MZero & \MQ_{01} & \dots & \MQ_{0N} \\
\hline
\MQ_{01} & \MQ_{11} & \dots & \MZero \\
\vdots & \vdots & \ddots & \vdots \\
\MQ_{0N} & \MZero & \dots & \MQ_{NN}
\emat. \label{eq:matrixCompactQ}
\eea
With cost matrix $\MQ$, and using the cyclic property of the trace operator, the \QCQP in eq.~\eqref{eq:TLSBinaryClone} can be written compactly as in the following proposition.
\begin{proposition}[Primal \QCQP] \label{prop:primalQCQP}
The \QCQP in eq.~\eqref{eq:TLSBinaryClone} is equivalent to the following \QCQP:
\bea \label{eq:qcqpforLagrangian}
(P)\quad \min_{\vxx \in \Real{4(N+1)}} & \trace{\MQ \vxx \vxx\tran} \\
\subject & \trace{\vxx_q \vxx_q\tran} = 1 \nonumber \\
& \vxx_{q_i} \vxx_{q_i}\tran = \vxx_{q} \vxx_{q}\tran, \forall i=1,\dots,N \nonumber
\eea
We call this \QCQP the \emph{primal problem} (P).
\end{proposition}

% Using the method of Lagrangian multipliers, 
The proposition can be proven by inspection.
We now introduce the \emph{Lagrangian function}~\cite{Boyd04book} of the primal ($P$).
\begin{proposition}[Lagrangian of Primal \QCQP]\label{prop:LagrangianPrimalQCQP}
The Lagrangian function of ($P$) can be written as:
\bea
& \calL(\vxx,\mu,\MLambda)=\trace{\MQ\vxx\vxx\tran}-\mu(\trace{\MJ\vxx\vxx\tran}-1) \nonumber \\
& - \sumAllPointsi \trace{\MLambda_i \vxx\vxx\tran} \label{eq:LagrangianNaive0}\\
& = \trace{(\MQ - \mu\MJ - \MLambda) \vxx\vxx\tran} + \mu. \label{eq:LagrangianNaive}
\eea
where $\MJ$ is a sparse matrix with all zeros except the first $4\times 4$ diagonal block being identity matrix:
\bea \label{eq:matrixJ}
\MJ = \bmat{c|ccc}
\eye_4 & \MZero & \cdots & \MZero \\
\hline
\MZero & \MZero & \cdots & \MZero \\
\vdots & \vdots & \ddots & \vdots \\
\MZero & \MZero & \cdots & \MZero
\emat,
\eea
and each $\MLambda_i,i=1,\dots,N$ is a sparse Lagrangian multiplier matrix with all zeros except two diagonal sub-blocks $\pm \MLambda_{ii} \in \sym^{4\times 4}$ (symmetric $4\times4$ matrices):
\bea \label{eq:matrixLambdai}
\MLambda_i = 
\bmat{c|ccccc} 
\MLambda_{ii} & \MZero & \cdots & \MZero & \cdots & \MZero \\
\hline
\MZero & \MZero & \cdots & \MZero & \cdots & \MZero \\
\vdots & \vdots & \ddots & \vdots & \ddots & \vdots\\
\MZero & \MZero & \cdots & -\MLambda_{ii} & \cdots & \MZero \\
\vdots & \vdots & \ddots & \vdots & \ddots & \vdots\\
\MZero & \MZero & \cdots & \MZero & \cdots & \MZero
\emat,
\eea
and $\MLambda$ is the sum of all $\MLambda_i$'s, $i=1,\dots,N$:
\bea \label{eq:matrixLambda}
& \displaystyle \MLambda=\sumAllPointsi \MLambda_i = \nonumber \\
& \hspace{-8mm} \bmat{c|ccccc} 
\sum\limits_{i=1}^N \MLambda_{ii} & \MZero & \dots & \MZero & \dots & \MZero \\
\hline
\MZero & -\MLambda_{11} & \dots & \MZero & \dots & \MZero \\
\vdots & \vdots & \ddots & \vdots & \ddots & \vdots\\
\MZero & \MZero & \dots & -\MLambda_{ii} & \dots & \MZero \\
\vdots & \vdots & \ddots & \vdots & \ddots & \vdots\\
\MZero & \MZero & \dots & \MZero & \dots & -\MLambda_{NN}
\emat.
\eea
\end{proposition}
\begin{proof}
The sparse matrix $\MJ$ defined in~\eqref{eq:matrixJ} satisfies $\trace{\MJ \vxx \vxx\tran} = \trace{\vxx_q \vxx_q\tran}$. Therefore $\mu (\trace{\MJ \vxx\vxx\tran}-1)$ is the same as $\mu ( \trace{\vxx_q \vxx_q\tran} - 1)$, and $\mu$ is the Lagrange multiplier associated to the constraint $\trace{\vxx_q \vxx_q\tran} = 1$ in ($P$). 
%
Similarly, from the definition of the matrix $\MLambda_i$ in~\eqref{eq:matrixLambda}, 
it follows:
\bea
\trace{\MLambda_i \vxx\vxx\tran} = \trace{\MLambda_{ii} (\vxx_{q_i}\vxx_{q_i}\tran - \vxx_q \vxx_q\tran)},
\eea
where $\MLambda_{ii}$ is the Lagrange multiplier (matrix) associated to each of the constraints $\vxx_{q_i}\vxx_{q_i}\tran = \vxx_q \vxx_q\tran$ in ($P$).
% $\trace{\MLambda_i \vxx \vxx\tran}=0$ implies the leading $4\times 4$ diagonal sub-block of $\vxx\vxx\tran$ is equal to the $(i+1)$-th $4 \times 4$ diagonal sub-block of $\vxx\vxx\tran$,\ie, $\vxx_{q_i}\vxx_{q_i}\tran = \vxx_q \vxx_q\tran$, corresponding to the second set of constraints in~\eqref{eq:qcqpforLagrangian}.
This proves that~\eqref{eq:LagrangianNaive0} (and eq.~\eqref{eq:LagrangianNaive}, which rewrites~\eqref{eq:LagrangianNaive0} in compact form) is the Lagrangian function of ($P$).
\end{proof}


From the expression of the Lagrangian, we can readily obtain the Lagrangian \emph{dual} problem.

\begin{proposition}[Lagrangian Dual of Primal \QCQP]\label{prop:LagrangianDualPrimal}
The following SDP is the Lagrangian dual for the primal \QCQP (P) in eq.~\eqref{eq:qcqpforLagrangian}:
\bea \label{eq:LagrangianDualNaive}
(D)\quad \max_{\substack{\mu \in \Real{} \\ \MLambda \in \Real{4(N+1)\times 4(N+1)}} } & \mu \\
\subject & \MQ - \mu\MJ - \MLambda \succeq 0 \nonumber 
\eea
where $\MJ$ and $\MLambda$ satisfy the structure in eq.~\eqref{eq:matrixJ} and~\eqref{eq:matrixLambda}.
\end{proposition}

\begin{proof}
By definition, the dual problem is~\cite{Boyd04book}:
\bea
\hspace{-3mm}\max_{\mu,\MLambda}\min_{\vxx}\calL(\vxx,\mu,\MLambda), 
\eea
where $\calL(\vxx,\mu,\MLambda)$ is the Lagrangian function. We observe:
% we can observe the (unrestricted) optimum of the Lagrangian function is:
\bea
\hspace{-3mm}\max_{\mu,\MLambda}\min_{\vxx}\calL(\vxx,\mu,\MLambda) = \begin{cases}
\mu & \text{if } \MQ - \mu\MJ - \MLambda \succeq 0 \\
-\infty & \text{otherwise}
\end{cases}.
\eea
Since we are trying to maximize the Lagrangian (with respect to the dual variables), we discard the case 
leading to a cost of $-\infty$, obtaining the dual problem in~\eqref{eq:LagrangianDualNaive}.
% Therefore we write the Lagrangian dual of ($P$) as in~\eqref{eq:LagrangianDualNaive}, concluding the proof.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
To connect the Lagrangian dual ($D$) to the naive SDP relaxation~\eqref{eq:naiveRelaxation} in Proposition~\ref{prop:naiveRelax}, we notice that the naive SDP relaxation is the dual SDP of the Lagrangian dual ($D$).
\begin{proposition}[Naive Relaxation is the Dual of the Dual]\label{prop:naiveRelaxIsDualofLagrangianDual}
The following SDP is the dual of the Lagrangian dual (D) in~\eqref{eq:LagrangianDualNaive}:
\bea
(DD)\quad \min_{\MZ \succeq 0}  & \trace{\MQ \MZ} \\
\subject  & \trace{[\MZ]_{qq}} = 1 \nonumber \\
& [\MZ]_{q_i q_i} = [\MZ]_{qq}, \forall i=1,\dots,N \nonumber
\eea
and (DD) is the same as the naive SDP relaxation in~\eqref{eq:naiveRelaxation}.
\end{proposition}
%
\begin{proof} 
We derive the Lagrangian dual problem of $(DD)$ and show that it is indeed ($D$) (see similar example in~\cite[p. 265]{Boyd04book}). Similar to the proof of Proposition~\eqref{prop:LagrangianPrimalQCQP}, we can associate Lagrangian multiplier $\mu\MJ$ (eq.~\eqref{eq:matrixJ}) to the constraint $\trace{[\MZ]_{qq}}=1$, and associate $\MLambda_i,i=1,\dots,N$ (eq.~\eqref{eq:matrixLambdai}) to constraints $[\MZ]_{q_i q_i} = [\MZ]_{qq},i=1,\dots,N$. In addition, we can associate matrix $\MTheta \in \sym^{4(N+1)\times 4(N+1)}$ to the constraint $\MZ \succeq 0$. Then the Lagrangian of the SDP ($DD$) is:
\bea
& \calL(\MZ,\mu,\MLambda,\MTheta)  \nonumber \\
& \hspace{-5mm}= \trace{\MQ \MZ} - \mu(\trace{\MJ \MZ} - 1) - \sum\limits_{i=1}^N (\trace{\MLambda_i \MZ}) - \trace{\MTheta \MZ} \nonumber \\
& = \trace{(\MQ - \mu \MJ - \MLambda - \MTheta) \MZ} + \mu,
\eea
and by definition, the dual problem is:
\bea
\max_{\mu,\MLambda,\MTheta}\min_{\MZ} \calL(\MZ,\mu,\MLambda,\MTheta).
\eea
Because:
\bea
\max_{\mu,\MLambda,\MTheta}\min_{\MZ} \calL = \begin{cases}
\mu & \text{if } \MQ - \mu\MJ - \MLambda - \MTheta \succeq 0 \\
-\infty & \text{otherwise}
\end{cases},
\eea
we can get the Lagrangian dual problem of ($DD$) is:
\bea \label{eq:LagrangianDualofDD}
\max_{\mu,\MLambda,\MTheta} & \mu \\
\subject & \MQ - \mu\MJ - \MLambda \succeq \MTheta \nonumber \\
& \MTheta \succeq 0 \nonumber 
\eea
Since $\MTheta$ is independent from the other decision variables and the cost function, we inspect that setting $\MTheta = \zero$ actually maximizes $\mu$ and therefore can be removed. Removing $\MTheta$ from~\eqref{eq:LagrangianDualofDD} indeed leads to ($D$) in eq.~\eqref{eq:LagrangianDualNaive}.
\end{proof}

We can also verify weak duality by the following calculation. Denote $f_{DD}=\trace{\MQ\MZ}$ and $f_D=\mu$. Recalling the structure of $\MLambda$ from eq.~\eqref{eq:matrixLambda}, we have $\trace{\MLambda \MZ}  = 0 $ because $[\MZ]_{q_i q_i}=[\MZ]_{qq},\forall i=1,\dots,N$. Moreover, we have $\mu=\mu\trace{\MJ \MZ}$ due to the pattern of $\MJ$ from eq.~\eqref{eq:matrixJ} and $\trace{[\MZ]_{qq}}=1$. Therefore, the following inequality holds:
\bea \label{eq:weakDualitySDP}
& f_{DD}-f_D=\trace{\MQ\MZ} - \mu \nonumber \\
& = \trace{\MQ\MZ} - \mu\trace{\MJ \MZ} - \trace{\MLambda \MZ} \nonumber \\
& = \trace{(\MQ-\mu\MJ-\MLambda)\MZ} \geq 0
\eea
where the last inequality holds true because both $\MQ-\mu\MJ-\MLambda$ and $\MZ$ are positive semidefinite matrices. Eq.~\eqref{eq:weakDualitySDP} shows $f_{DD} \geq f_D$ always holds inside the feasible set and therefore by construction of ($P$), ($D$) and ($DD$), we have the following \emph{weak duality} relation:
\bea \label{eq:weakDualityByConstruction}
f^\star_D \leq f^\star_{DD} \leq f^\star_P.
\eea
where the first inequality follows from eq.~\eqref{eq:weakDualitySDP} and the second inequality originates from the point that ($DD$) is a convex relaxation of ($P$), which has a larger feasible set and therefore the optimal cost of ($DD$) ($f^\star_{DD}$) is always smaller than the optimal cost of ($P$) ($f^\star_P$).

\subsection{KKT conditions and strong duality}
\label{sec:KKTStrongDuality}
Despite the fact that weak duality gives lower bounds for objective of the primal \QCQP ($P$), in this context we are interested in cases when \emph{strong duality} holds, \ie:
\bea \label{eq:strongdualityDef}
f^\star_D = f^\star_{DD} = f^\star_P,
\eea
since in these cases solving any of the two convex SDPs ($D$) or ($DD$) will also solve the original non-convex \QCQP ($P$) to \emph{global optimality}.

Before stating the main theorem for strong duality, we study the \emph{Karush-Kuhn-Tucker} (KKT) conditions~\cite{Boyd04book} for the primal \QCQP ($P$) in~\eqref{eq:qcqpforLagrangian}, which will help pave the way to study strong duality.
\begin{proposition}[KKT Conditions for Primal \QCQP]\label{prop:KKTForPrimalQCQP}
If $\vxx^\star$ is an optimal solution to the primal \QCQP ($P$) in~\eqref{eq:qcqpforLagrangian} (also~\eqref{eq:TLSBinaryClone}), and let $(\mu^\star,\MLambda^\star)$ be the corresponding optimal dual variables (maybe not unique), then it must satisfy the following KKT conditions:
\bea
& \expl{Stationary condition} 
& \label{eq:KKTStationary}(\MQ - \mu^\star \MJ - \MLambda^\star) \vxx^\star = \zero, \\
& \expl{Primal feasibility condition} 
& \label{eq:KKTFeasibility} \vxx^\star \text{ satisfies the constraints in~\eqref{eq:qcqpforLagrangian} }.
\eea
\end{proposition}
Using Propositions~\ref{prop:primalQCQP}-\ref{prop:KKTForPrimalQCQP}, we state the following theorem that provides a sufficient condition for strong duality. % in~\eqref{eq:strongdualityDef} holds.
\begin{theorem}[Sufficient Condition for Strong Duality]\label{thm:generalStrongDuality}
Given a stationary point $\vxx^\star$, if there exist dual variables $(\mu^\star,\MLambda^\star)$ (maybe not unique) such that $(\vxx^\star,\mu^\star,\MLambda^\star)$ satisfy both the KKT conditions in Proposition~\ref{prop:KKTForPrimalQCQP} and the dual feasibility condition $\MQ - \mu^\star\MJ - \MLambda^\star \succeq 0$ in Proposition~\ref{prop:LagrangianDualPrimal}, then:
\begin{enumerate}[label=(\roman*)]
\item \label{item:strongDuality1} There is no duality gap between (P), (D) and (DD), \ie $f^\star_{P}=f^\star_{D}=f^\star_{DD}$,
\item \label{item:strongDuality2} $\vxx^\star$ is a global minimizer for (P).
\end{enumerate}
Moreover, if we have $\rank{\MQ - \mu^\star\MJ - \MLambda^\star}=4(N+1)-1$, \ie, $\MQ - \mu^\star\MJ - \MLambda^\star$ has $4(N+1)-1$ strictly positive eigenvalues and only one zero eigenvalue, then we have the following:
\begin{enumerate}[resume,label=(\roman*)]
\item \label{item:strongDuality3} $\pm \vxx^\star$ are the two unique global minimizers for (P),
\item \label{item:strongDuality4} The optimal solution to (DD), denoted as $\MZ^\star$, has rank 1 and can be written as $\MZ^\star=(\vxx^\star)(\vxx^\star)\tran$.
\end{enumerate}
\end{theorem}
\begin{proof}
Recall from eq.~\eqref{eq:weakDualityByConstruction} that we already have weak duality by construction of ($P$), ($D$) and ($DD$). Now since $(\vxx^\star,\mu^\star,\MLambda^\star)$ satisfies the KKT conditions~\eqref{eq:KKTFeasibility} and~\eqref{eq:KKTStationary}, we have:
\bea
& (\MQ - \mu^\star \MJ - \MLambda^\star)\vxx^\star = \zero \Rightarrow \nonumber \\
& (\vxx^\star)\tran(\MQ - \mu^\star\MJ - \MLambda^\star)(\vxx^\star) = 0 \Rightarrow \\
& \hspace{-8mm}(\vxx^\star)\tran \MQ (\vxx^\star) = \mu^\star (\vxx^\star)\tran \MJ (\vxx^\star) + (\vxx^\star)\tran \MLambda^\star (\vxx^\star) \Rightarrow \\
& \expl{$\vxstar$ satisfies the constraints in ($P$) by KKT~\eqref{eq:KKTFeasibility}}
& \expl{Recall structural partition of $\MJ$ and $\MLambda$ in~\eqref{eq:matrixJ} and~\eqref{eq:matrixLambda}}
& \trace{\MQ (\vxstar)(\vxstar)\tran} = \mu^\star,
\eea
which shows the cost of ($P$) is equal to the cost of ($D$) at $(\vxstar, \mu^\star, \MLambda^\star)$. Moreover, since $\MQ - \mu^\star\MJ - \MLambda^\star \succeq 0$ means $(\mu^\star,\MLambda^\star)$ is actually dual feasible for ($D$), hence we have strong duality between ($P$) and ($D$):
$f^\star_P = f^\star_D$. Because $f^\star_{DD}$ is sandwiched between $f^\star_P$ and $f^\star_D$ according to~\eqref{eq:weakDualityByConstruction}, we have indeed strong duality for all of them:
\bea
f^\star_D = f^\star_{DD} = f^\star_P,
\eea
proving~\ref{item:strongDuality1}. To prove~\ref{item:strongDuality2}, we observe that for any $\vxx \in \Real{4(N+1)}$, $\MQ - \mu^\star\MJ - \MLambda^\star \succeq 0$ means:
\bea
\vxx\tran (\MQ - \mu^\star\MJ - \MLambda^\star) \vxx \geq 0.
\eea
Specifically, let $\vxx$ be any vector that lies inside the feasible set of ($P$), \ie, $\trace{\vxx_q \vxx_q\tran}=1$ and $\vxx_{q_i}\vxx_{q_i}\tran = \vxx_q \vxx_q\tran,\forall i=1,\dots,N$, then we have:
\bea
& \vxx\tran (\MQ - \mu^\star\MJ - \MLambda^\star) \vxx \geq 0 \Rightarrow \nonumber \\
& \vxx\tran \MQ \vxx \geq \mu^\star \vxx\tran \MJ \vxx + \vxx\tran \MLambda^\star \vxx \Rightarrow \\
& \trace{\MQ \vxx \vxx\tran} \geq \mu^\star = \trace{\MQ (\vxstar)(\vxstar)\tran},
\eea
showing that the cost achieved by $\vxstar$ is no larger than the cost achieved by any other vectors inside the feasible set, which means $\vxstar$ is indeed a global minimizer to ($P$).

Next we use the additional condition of $\rank{\MQ - \mu^\star\MJ - \MLambda^\star}=4(N+1)-1$ to prove $\pm \vxstar$ are the two unique global minimizers to ($P$). Denote $\MM^\star=\MQ - \mu^\star\MJ - \MLambda^\star$, since $\MM^\star$ has only one zero eigenvalue with associated eigenvector $\vxstar$ (\cf KKT condition~\eqref{eq:KKTStationary}), its nullspace is defined by $\ker(\MM^\star) = \{\vxx \in \Real{4(N+1)}: \vxx = a \vxstar ,a\in \Real{} \}$. Now denote the feasible set of ($P$) as $\Omega(P)$. It is clear to see that any vector in $\Omega(P)$ is a vertical stacking of $N+1$ unit quaternions and thus must have 2-norm equal to $\sqrt{N+1}$. Since $\vxstar \in \Omega(P)$ is already true, in order for any vector $\vxx=a\vxstar$ in $\ker(\MM^\star)$ to be in $\Omega(P)$ as well, it must hold $|a|\Vert \vxx \Vert = \sqrt{N+1}$ and therefore $a=\pm 1$, \ie, $\ker(\MM^\star)\cap \Omega(P) = \{\pm\vxstar \}$. With this observation, we can argue that for any $\vxx$ inside $\Omega(P)$ that is not equal to $\{\pm \vxstar \}$, $\vxx$ cannot be in $\ker(\MM^\star)$ and therefore:
\bea
& \vxx\tran (\MM^\star) \vxx > 0 \Rightarrow \\
& \vxx\tran \MQ \vxx > \mu^\star \vxx\tran \MJ \vxx + \vxx\tran \MLambda^\star \vxx \Rightarrow \\
& \trace{\MQ \vxx \vxx\tran} > \mu^\star = \trace{\MQ(\vxstar)(\vxstar)\tran},
\eea
which means for any vector $\vxx \in \Omega(P)/ \{\pm \vxstar \} $, it results in strictly higher cost than $\pm \vxstar$. Hence $\pm \vxstar$ are the two unique global minimizers to ($P$) and~\ref{item:strongDuality3} is true.

To prove~\ref{item:strongDuality4}, notice that since strong duality holds and $f^\star_{DD}=f^\star_D$, we can write the following according to eq.~\eqref{eq:weakDualitySDP}:
\bea \label{eq:strongDualitySDP}
\trace{(\MQ - \mu^\star \MJ - \MLambda^\star) \MZ^\star} = 0.
\eea
Since $\MM^\star = \MQ - \mu^\star \MJ - \MLambda^\star \succeq 0$ and has rank $4(N+1)-1$, we can write $\MM^\star = \barM\tran \barM$ with $\barM \in \Real{(4(N+1)-1) \times 4(N+1)}$ and $\rank{\barM} = 4(N+1)-1$. Similarly, we can write $\MZ^\star = \barZ \barZ\tran$ with $\barZ \in \Real{4(N+1) \times r}$ and $\rank{\barZ}=r=\rank{\MZ^\star}$. Then from~\eqref{eq:strongDualitySDP} we  have:
\bea
& \trace{\MM^\star \MZ^\star} = \trace{\barM\tran \barM \barZ \barZ\tran} \nonumber \\
& = \trace{\barZ\tran\barM\tran \barM\barZ} = \trace{(\barM\barZ)\tran (\barM \barZ)} \nonumber \\
& = \Vert \barM \barZ \Vert_F^2 = 0,
\eea
which gives us $\barM \barZ = \zero$. Using the rank inequality $\rank{\barM \barZ} \geq \rank{\barM} + \rank{\barZ} - 4(N+1)$, we have:
\bea
& 0 \geq 4(N+1)-1 + r - 4(N+1) \Rightarrow \nonumber \\
& r \leq 1.
\eea
Since $\barZ \neq \zero$, we conclude that $\rank{\MZ^\star} = \rank{\barZ}=r=1$. As a result, since $\rank{\MZ^\star} = 1$, and the rank constraint was the only constraint we dropped when relaxing the \QCQP ($P$) to SDP ($DD$), we conclude that the relaxation is indeed tight. In addition, the rank 1 decomposition $\barZ$ of $\MZ^\star$ is also the global minimizer to ($P$). However, from~\ref{item:strongDuality3}, we know there are only two global minimizers to ($P$): $\vxstar$ and $-\vxstar$, so $\barZ \in \{\pm \vxstar\}$. Since the sign is irrelevant, we can always write $\MZ^\star = (\vxstar) (\vxstar)\tran$, concluding the proof for~\ref{item:strongDuality4}. 
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Strong duality in noiseless and outlier-free case}
\label{sec:strongDualityNoiselessOutlierfree}

Now we are ready to prove Theorem~\ref{thm:strongDualityNoiseless} using Theorem~\ref{thm:generalStrongDuality}. To do so, we will show that in the noiseless and outlier-free case, it is always possible to construct $\mu^\star$ and $\MLambda^\star$ from $\vxstar$ and $\MQ$ such that $(\vxstar,\mu^\star,\MLambda^\star)$ satisfies the KKT conditions, and the dual matrix $\MM^\star = \MQ - \mu^\star\MJ - \MLambda^\star$ is positive semidefinite and has only one zero eigenvalue. 

\myParagraph{Preliminaries} When there are no noise and outliers in the measurements, \ie, $\vb_i = \MR \va_i, \forall i=1,\dots,N$, we have $\Vert \vb_i \Vert^2 = \Vert \va_i \Vert^2,\forall i=1,\dots,N$. Moreover, without loss of generality, we assume $\sigma_i^2=1$ and $\barcsq > 0$. 
%(note that $\sigma_i^2=1$ makes sense in eq.~\eqref{eq:TLSWahbaRot} and we do not take $\sigma_i^2=0$). 
With these assumptions, we simplify the blocks $\MQ_{0i}$ and $\MQ_{ii}$ in the matrix $\MQ$, \cf~\eqref{eq:matrixCompactQ} and~\eqref{eq:costInQuadraticFormBeforeLifting}:
\bea
& \label{eq:simplifiedQ0i} \MQ_{0i} = \frac{\Vert \va_i \Vert^2}{2}\eye_4 + \frac{\MOmega_1(\hatvb_i) \MOmega_2(\hatva_i)}{2} - \frac{\barcsq}{4}\eye_4,\\
& \label{eq:simplifiedQii} \MQ_{ii} = \Vert \va_i \Vert^2 \eye_4 + \MOmega_1(\hatvb_i)\MOmega_2(\hatva_i) + \frac{\barcsq}{2}\eye_4.
\eea


Due to the primal feasibility condition~\eqref{eq:KKTFeasibility}, we know $\vxx^\star$ can be written as $N+1$ quaternions (\cf proof of~\eqref{eq:equivalentConstraints}): $\vxx^\star= [(\vq^\star)\tran\ \theta_1^\star (\vq^\star)\tran\ \dots\ \theta_N^\star(\vq^\star)\tran]\tran$, where each $\theta_i^\star$ is a binary variable in $\{-1,+1\}$. Since we have assumed no noise and no outliers, we know $\theta_i^\star=+1$ for all $i$'s and therefore $\vxx^\star= [(\vq^\star)\tran\ (\vq^\star)\tran\ \dots\ (\vq^\star)\tran]\tran$. We can write the KKT stationary condition in matrix form as:
\bea \label{eq:KKTStationaryMatrixForm}
\hspace{-7mm}\overbrace{ \bmat{c|ccc}
\substack{-\mu^\star \eye_4 - \\ \sum\limits_{i=1}^N\MLambda^\star_{ii} }& \MQ_{01} & \dots & \MQ_{0N} \\
\hline
\MQ_{01} & {\scriptstyle \MQ_{11}+\MLambda^\star_{11} } & \dots & \MZero \\
\vdots & \vdots & \ddots & \vdots \\
\MQ_{0N} & \MZero & \dots & {\scriptstyle \MQ_{NN}+\MLambda^\star_{NN}}
\emat}^{\MM^\star = \MQ - \mu^\star\MJ - \MLambda^\star}
\overbrace{ \bmat{c}
\vq^\star \\
\hline
\vq^\star \\
\vdots \\
\vq^\star
\emat}^{\vxstar} = \zero \nonumber \hspace{-8mm}\\\hspace{-8mm}
\eea
and we index the block rows of $\MM^\star$ from top to bottom as $0,1,\dots,N$. The first observation we make is that eq.~\eqref{eq:KKTStationaryMatrixForm} is a (highly) under-determined linear system with respect to the dual variables $(\mu^\star,\MLambda^\star)$, because the linear system has $10N+1$ unknowns  (each symmetric $4\times4$ matrix $\MLambda^\star_{ii}$ has 10 unknowns, plus one unknown from $\mu^\star$), but only has $4(N+1)$ equations. To expose the structure of the linear system, we will apply a similarity transformation to the matrix $\MM^\star$. Before we introduce the similarity transformation, we need additional properties about quaternions, described in the Lemma below. The properties can be proven by inspection.

\begin{lemma}[More Quaternion Properties]\label{lemma:quaternionProperties}
The following properties about unit quaternions, involving the linear operators $\MOmega_1(\cdot)$ and $\MOmega_2(\cdot)$ introduced in eq.~\eqref{eq:Omega_1} hold true: 
%We will use them without proof, the interested readers are suggested to verify these properties on their own.
\begin{enumerate}[label=(\roman*)]
\item \label{item:commutativeOmega} Commutative: for any two vectors $\vxx,\vy \in \Real{4}$, The following equalities hold:
\bea \label{eq:commutativeOmega}
\MOmega_1(\vxx)\MOmega_2(\vy) = \MOmega_2(\vy)\MOmega_1(\vxx); \\
\MOmega_1(\vxx)\MOmega_2\tran(\vy) = \MOmega_2\tran(\vy)\MOmega_1(\vxx); \\
\MOmega_1\tran(\vxx)\MOmega_2(\vy) = \MOmega_2(\vy)\MOmega_1\tran(\vxx); \\
\MOmega_1\tran(\vxx)\MOmega_2\tran(\vy) = \MOmega_2\tran(\vy)\MOmega_1\tran(\vxx). 
\eea
\item \label{item:orthogonality} Orthogonality: for any unit quaternion $\vq \in \calS^3$, $\MOmega_1(\vq)$ and $\MOmega_2(\vq)$ are orthogonal matrices:
\bea
\MOmega_1(\vq)\MOmega_1\tran(\vq) = \MOmega_1\tran(\vq)\MOmega_1(\vq) = \eye_4; \\
\MOmega_2(\vq)\MOmega_1\tran(\vq) = \MOmega_2\tran(\vq)\MOmega_1(\vq) = \eye_4.
\eea
\item \label{item:rotateqtoe} For any unit quaternion $\vq \in \calS^3$, the following equalities hold:
\bea
\MOmega_1\tran(\vq)\vq = \MOmega_2\tran(\vq)\vq = [0,0,0,1]\tran.
\eea
\item \label{item:OmegaandR} For any unit quaternion $\vq \in \calS^3$, denote $\MR$ as the unique rotation matrix associated with $\vq$, then the following equalities hold:
\bea
\hspace{-10mm} \MOmega_1(\vq)\MOmega_2\tran(\vq)=\MOmega_2\tran(\vq)\MOmega_1(\vq)=\bmat{cc} \MR & \zero \\ \zero & 1 \emat \doteq \tilde{\MR}; \\
\hspace{-10mm} \MOmega_2(\vq)\MOmega_1\tran(\vq) = \MOmega_1\tran(\vq)\MOmega_2(\vq) = \bmat{cc} \MR\tran & \zero \\ \zero & 1 \emat \doteq \tilde{\MR}\tran.
\eea
\end{enumerate}
\end{lemma}

\myParagraph{Rewrite dual certificates using similarity transform}
Now we are ready to define the similarity transformation. We define the matrix $\MD \in \Real{4(N+1)\times 4(N+1)}$ as the following block diagonal matrix:
\bea
& \MD = \bmat{cccc}
\MOmega_1(\vq^\star) & \zero & \cdots & \zero \\
\zero & \MOmega_1(\vq^\star) & \cdots & \zero \\
\vdots & \vdots & \ddots & \vdots \\
\zero & \zero & \cdots & \MOmega_1(\vq^\star)
\emat.
\eea
% where the $\kron$ here denotes the matrix Kronecker product (not the quaternion product). 
It is obvious to see that $\MD$ is an orthogonal matrix from~\ref{item:orthogonality} in Lemma~\ref{lemma:quaternionProperties}, \ie, $\MD\tran \MD = \MD \MD\tran = \eye_{4(N+1)}$. Then we have the following Lemma.
\begin{lemma}[Similarity Transformation]\label{lemma:similarityTransform}
Define $\MN^\star \doteq \MD\tran \MM^\star \MD$, then:
\begin{enumerate}[label=(\roman*)]
\item \label{item:sameEigenvalues} $\MN^\star$ and $\MM^\star$ have the same eigenvalues, and
\bea
\hspace{-5mm}\MM^\star \succeq 0 \Leftrightarrow \MN^\star \succeq 0,\ \rank{\MM^\star}=\rank{\MN^\star}.
\eea
\item \label{item:rotatedq} Define $\ve = [0,0,0,1]\tran$ and $\vr = [\ve\tran\ \ve\tran\ \dots\ \ve\tran]\tran$ as the vertical stacking of $N+1$ copies of $\ve$, then:
\bea
\MM^\star \vxstar=\zero \Leftrightarrow \MN^\star \vr = \zero.
\eea
\end{enumerate}
\end{lemma}
\begin{proof} Because $\MD\tran \MD = \eye_{4(N+1)}$, we have $\MD\tran = \MD\inv$ and $\MN^\star = \MD\tran \MM^\star \MD = \MD\inv \MM\tran \MD$ is similar to $\MM^\star$. Therefore, by matrix similarity, $\MM^\star$ and $\MN^\star$ have the same eigenvalues, and $\MM^\star$ is positive semidefinite if and only if $\MN^\star$ is positive semidefinite~\cite[p. 12]{Boyd06notes}. To show~\ref{item:rotatedq}, we start by pre-multiplying both sides of eq.~\eqref{eq:KKTStationaryMatrixForm} by $\MD\tran$:
\bea
& \MM^\star \vxstar =\zero \Leftrightarrow \MD\tran\MM^\star \vxstar = \MD\tran \zero \Leftrightarrow \\
& \expl{$\MD \MD\tran=\eye_{4(N+1)}$}
& \MD\tran\MM^\star (\MD \MD\tran) \vxstar = \zero \Leftrightarrow \\
& (\MD\tran\MM^\star\MD)(\MD\tran\vxstar) = \zero \Leftrightarrow \\
& \expl{$\MOmega_1\tran(\vq^\star) \vq^\star = \ve$ from~\ref{item:rotateqtoe} in Lemma~\ref{lemma:quaternionProperties}}
& \MN^\star \vr = \zero, \label{eq:KKTStationaryN}
\eea
concluding the proof.
\end{proof}
Lemma~\ref{lemma:similarityTransform} suggests that constructing $\MM^\star \succeq 0$ and $\rank{\MM^\star}=4(N+1)-1$ that satisfies the KKT conditions~\eqref{eq:KKTStationary} is equivalent to constructing $\MN^\star \succeq 0$ and $\rank{\MN^\star}=4(N+1)-1$ that satisfies~\eqref{eq:KKTStationaryN}. We then study the structure of $\MN^\star$ and rewrite the KKT stationary condition.

\myParagraph{Rewrite KKT conditions}
In noiseless and outlier-free case, the KKT condition $\MM^\star \vxstar = \zero$ is equivalent to $\MN^\star\vr =\zero$. Formally, after the similarity transformation $\MN^\star = \MD\tran \MM^\star \MD$, the KKT conditions can be explicitly rewritten as in the following proposition.

\begin{proposition}[KKT conditions after similarity transformation]
The KKT condition $\MN^\star \vr = \zero$ (which is equivalent to eq.~\eqref{eq:KKTStationaryMatrixForm}) can be written in matrix form:
\bea \label{eq:KKTStationaryMatrixFormInN}
\hspace{-8mm}\bmat{c|ccc}
 {\scriptstyle -\sum\limits_{i=1}^N\barLambda^\star_{ii} } & \barMQ_{01} & \dots & \barMQ_{0N} \\
\hline
\barMQ_{01} & {\scriptstyle \barMQ_{11}+\barLambda^\star_{11} } & \dots & \MZero \\
\vdots & \vdots & \ddots & \vdots \\
\barMQ_{0N} & \MZero & \dots & {\scriptstyle \barMQ_{NN}+\barLambda^\star_{NN}}
\emat
\bmat{c}
\ve \\
\hline 
\ve \\
\vdots \\
\ve
\emat = \zero.
\eea
with $\mu^\star = 0$ being removed compared to eq.~\eqref{eq:KKTStationaryMatrixForm} and $\barMQ_{0i}$ and $\barMQ_{ii},i=1,\dots,N$ are the following sparse matrices:
\bea
& \barMQ_{0i} \doteq \MOmega_1\tran(\vq^\star)\MQ_{0i}\MOmega_1(\vq^\star) \nonumber \\
& \hspace{-5mm} = \bmat{cc}
\left( \frac{\Vert \va_i \Vert^2}{2} - \frac{\barcsq}{4} \right) \eye_3 - \frac{ \vSkew{\va_i}^2}{2} - \frac{\va_i \va_i\tran}{2} & \zero \\
\zero & - \frac{\barcsq}{4}
\emat; \label{eq:barMQ0i}\\
& \barMQ_{ii} \doteq \MOmega_1\tran(\vq^\star)\MQ_{ii}\MOmega_1(\vq^\star) \nonumber \\
& \hspace{-5mm} = \bmat{cc}
\left( \Vert \va_i \Vert^2 + \frac{\barcsq}{2} \right)\eye_3 - \vSkew{\va_i}^2 - \va_i \va_i\tran & \zero \\
\zero & \frac{\barcsq}{2}
\emat, \label{eq:barMQii}
\eea
and $\barLambda_{ii}^\star \doteq \MOmega_1\tran(\vq^\star) \MLambda^\star_{ii} \MOmega_1(\vq^\star) $ has the following form:
\bea \label{eq:generalFormBarLambda}
\barLambda^\star_{ii} = \bmat{cc}
\ME_{ii} & \valpha_i \\
\valpha_i\tran & \lambda_i
\emat,
\eea
where $\ME_{ii} \in \sym^{3\times3}$,$\valpha_i \in \Real{3}$ and $\lambda_i \in \Real{}$.
\end{proposition}
\begin{proof}
We first prove that $\barMQ_{0i}$ and $\barMQ_{ii}$ have the forms in~\eqref{eq:barMQ0i} and~\eqref{eq:barMQii} when there are no noise and outliers in the measurements. Towards this goal, we examine the similar matrix to $\MOmega_1(\hatvb_i)\MOmega_2(\hatva_i)$ (as it is a common part to $\MQ_{0i}$ and $\MQ_{ii}$):
\bea
& \MOmega_1\tran(\vq^\star) \MOmega_1(\hatvb_i)\MOmega_2(\hatva_i) \MOmega_1(\vq^\star) \nonumber \\
& \expl{Commutative property in Lemma~\ref{lemma:quaternionProperties}~\ref{item:commutativeOmega}}
& = \MOmega_1\tran(\vq^\star) \MOmega_1(\hatvb_i) \MOmega_1(\vq^\star) \MOmega_2(\hatva_i) \\
& \expl{Orthogonality property in Lemma~\ref{lemma:quaternionProperties}~\ref{item:orthogonality}}
& \hspace{-5mm}= \MOmega_1\tran(\vq^\star) \MOmega_2(\vq^\star) \MOmega_2\tran(\vq^\star)  \MOmega_1(\hatvb_i) \MOmega_1(\vq^\star) \MOmega_2(\hatva_i) \\
& \expl{Lemma~\ref{lemma:quaternionProperties}~\ref{item:commutativeOmega} and~\ref{item:OmegaandR}}
& = (\tilde{\MR}^\star)\tran \MOmega_1(\hatvb_i)\MOmega_2\tran(\vq^\star)\MOmega_1(\vq^\star)\MOmega_2(\hatva_i) \\
& \expl{Lemma~\ref{lemma:quaternionProperties}~\ref{item:OmegaandR} }
& = (\tilde{\MR}^\star)\tran \MOmega_1(\hatvb_i) (\tilde{\MR}^\star) \MOmega_2(\hatva_i) \\
& = \bmat{cc}
(\MR^\star)\tran \vSkew{\vb_i}\MR^\star & (\MR^\star)\tran \vb_i \\
-\vb_i\tran \MR^\star & 0
\emat \MOmega_2(\hatva_i) \\
& = \bmat{cc}
\vSkew{\va_i} & \va_i \\
-\va_i\tran & 0 
\emat
\bmat{cc}
-\vSkew{\va_i} & \va_i \\
-\va_i\tran & 0
\emat \\
&=\bmat{cc}
-\vSkew{\va_i}^2-\va_i\va_i\tran & \zero \\
\zero & -\Vert \va_i \Vert^2
\emat.
\eea
Using this property, and recall the definition of $\MQ_{0i}$ and $\MQ_{ii}$ in eq.~\eqref{eq:simplifiedQ0i} and~\eqref{eq:simplifiedQii}, the similar matrices to $\MQ_{0i}$ and $\MQ_{ii}$ can be shown to have the expressions in~\eqref{eq:barMQ0i} and~\eqref{eq:barMQii} by inspection. 

Showing $\barLambda_{ii}$ having the expression in~\eqref{eq:generalFormBarLambda} is straightforward. Since $\MLambda_{ii}^\star$ is symmetric, $\barLambda_{ii}^\star= \MOmega_1\tran(\vq^\star) \MLambda^\star_{ii} \MOmega_1(\vq^\star)$ must also be symmetric and therefore eq.~\eqref{eq:generalFormBarLambda} must be true for some $\ME_{ii}$, $\valpha_i$ and $\lambda_i$.

Lastly, in the noiseless and outlier-free case, $\mu^\star$ is zero due to the following:
\bea
& \mu^\star = \trace{\MQ(\vxstar)(\vxstar)\tran} \nonumber \\
& \expl{Recall $\MQ$ from eq.~\eqref{eq:matrixCompactQ} }
& = (\vq^\star)\tran \left( \sumAllPointsi (\MQ_{ii} + 2\MQ_{0i}) \right) (\vq^\star) \\
& \hspace{-5mm}= (\vq^\star)\tran \left( 2 \sumAllPointsi \Vert \va_i \Vert^2 +  \MOmega_1(\hatvb_i)\MOmega_2(\hatva_i)  \right) (\vq^\star) \\
& \expl{Recall eq.~\eqref{eq:developQuatProduct}} 
& = 2 \sumAllPointsi \Vert \va_i \Vert^2 - \hatvb_i\tran (\vq^\star \kron \hatva_i \kron (\vq^\star)\inv) \\
& = 2 \sumAllPointsi \Vert \va_i \Vert^2 - \vb_i\tran (\MR^\star\va_i) \\
& = 2 \sumAllPointsi \Vert \va_i \Vert^2 - \| \vb_i \|^2 = 0.
\eea
concluding the proof.
\end{proof}

\myParagraph{From KKT condition to sparsity pattern of dual variable} From the above proposition about the rewritten KKT condition~\eqref{eq:KKTStationaryMatrixFormInN}, we can claim the following sparsity pattern on the dual variables $\barLambda_{ii}$.
\begin{lemma}[Sparsity Pattern of Dual Variables] \label{lemma:sparsityPatternDualVar}
The KKT condition eq.~\eqref{eq:KKTStationaryMatrixFormInN} holds if and only if the dual variables $\{\barLambda_{ii}\}_{i=1}^N$ have the following sparsity pattern:
\bea \label{eq:sparsityPatternLambda}
\barLambda^\star_{ii} = \bmat{cc}
\ME_{ii} & \zero_3 \\
\zero_3 & -\frac{\barcsq}{4}
\emat,
\eea
\ie, $\valpha_i=0$ and $\lambda_i = -\frac{\barcsq}{4}$ in eq.~\eqref{eq:generalFormBarLambda} for every $i=1,\dots,N$.
\end{lemma}
\begin{proof}
We first proof the trivial direction ($\Leftarrow$). If $\barLambda^\star_{ii}$ has the sparsity pattern in eq.~\eqref{eq:sparsityPatternLambda}, then the product of the $i$-th block row of $\MN^\star$ ($i=1,\dots,N$) and $\vr$ writes (\cf eq.~\eqref{eq:KKTStationaryMatrixFormInN}):
\bea
& \left( \barMQ_{0i} + \barMQ_{ii} + \barLambda_{ii}^\star \right) \ve \nonumber \\
& \expl{Recall $\barMQ_{0i}$ and $\barMQ_{ii}$ from eq.~\eqref{eq:barMQ0i} and~\eqref{eq:barMQii}}
& = \bmat{cc}
\star & \zero_3 \\
\zero_3 & 0
\emat \bmat{c}
\zero_3 \\ 1 \emat = \zero_4, \label{eq:KKTEveryRowVanish}
\eea
which is equal to $\zero_4$ for sure. For the product of the $0$-th block row (the very top row) of $\MN^\star$ and $\vr$, we get:
\bea
& \left( \sumAllPointsi\barMQ_{0i} - \barLambda_{ii}^\star \right)\ve \nonumber \\
& = \bmat{cc}
\star & \zero_3 \\
\zero_3 & 0
\emat \bmat{c}
\zero_3 \\ 1 \emat = \zero_4,
\eea
which vanishes as well. Therefore, $\barLambda^\star_{ii}$ having the sparsity pattern in eq.~\eqref{eq:sparsityPatternLambda} provides a sufficient condition for KKT condition in eq.~\eqref{eq:KKTStationaryMatrixFormInN}. To show the other direction ($\Rightarrow$), first notice that eq.~\eqref{eq:KKTStationaryMatrixFormInN} implies eq.~\eqref{eq:KKTEveryRowVanish} holds true for all $i=1,\dots,N$ and in fact, eq.~\eqref{eq:KKTEveryRowVanish} provides the following equation for constraining the general form of $\barLambda^\star_{ii}$ in eq.~\eqref{eq:generalFormBarLambda}:
\bea
& \left( \barMQ_{0i} + \barMQ_{ii} + \barLambda_{ii}^\star \right) \ve \nonumber \\
& = \bmat{cc}
\star & \valpha_i \\
\valpha_i\tran & \lambda_i + \frac{\barcsq}{4}
\emat \bmat{c}
\zero_3 \\ 1 \emat = \zero_4,
\eea
which directly gives rise to:
\bea
\begin{cases}
\valpha_i = \zero_3 \\
\lambda_i + \frac{\barcsq}{4} = 0
\end{cases}.
\eea
and the sparsity pattern in eq.~\eqref{eq:sparsityPatternLambda}, showing that $\barLambda^\star_{ii}$ having the sparsity pattern in eq.~\eqref{eq:sparsityPatternLambda} is also a necessary condition.
\end{proof}

\myParagraph{Find the dual certificate}
Lemma~\ref{lemma:sparsityPatternDualVar} further suggests that the linear system resulted from KKT conditions~\eqref{eq:KKTStationaryMatrixFormInN} (also~\eqref{eq:KKTStationaryMatrixForm}) is highly under-determined in the sense that we have full freedom in choosing the $\ME_{ii}$ block of the dual variable $\barLambda_{ii}^\star$. Therefore, we introduce the following proposition.

\begin{proposition}[Construction of Dual Variable]\label{prop:constructionDualVariable}
In the noiseless and outlier-free case, choosing $\ME_{ii}$ as:
\bea \label{eq:choiceOfE}
\ME_{ii} = \vSkew{\va_k}^2 - \frac{1}{4} \barcsq \eye_3, \forall i =1,\dots,N
\eea
and choosing $\barLambda^\star_{ii}$ as having the sparsity pattern in~\eqref{eq:sparsityPatternLambda} will not only satisfy the KKT conditions in~\eqref{eq:KKTStationaryMatrixFormInN} but also make $\MN^\star \succeq 0$ and $\rank{\MN^\star}=4(N+1)-1$. Therefore, by Theorem~\ref{thm:generalStrongDuality}, the naive relaxation in Proposition~\ref{prop:naiveRelax} is always tight and Theorem~\ref{thm:strongDualityNoiseless} is true.
\end{proposition}
\begin{proof}
By Lemma~\ref{lemma:sparsityPatternDualVar}, we only need to prove the choice of $\ME_{ii}$ in~\eqref{eq:choiceOfE} makes $\MN^\star \succeq 0$ and $\rank{\MN^\star}=4(N+1)-1$. Towards this goal, we will show that for any vector $\vu \in \Real{4(N+1)}$, $\vu\tran \MN^\star \vu \geq 0$ and the nullspace of $\MN^\star$ is $\ker(\MN^\star)=\{\vu: \vu = a\vr, a\in \Real{} \text{ and } a\neq 0\}$ ($\MN^\star$ has a single zero eigenvalue with associated eigenvector $\vr$). We partition $\vu = [\vu_0\tran\ \vu_1\tran\ \dots\ \vu_N\tran]\tran$, where $\vu_i \in \Real{4},\forall i=0,\dots,N$. Then using the form of $\MN^\star$ in~\eqref{eq:KKTStationaryMatrixFormInN}, we can write $\vu\tran \MN^\star \vu$ as:
\bea
& \vu\tran \MN^\star \vu = - \sumAllPointsi \vu_0\tran \barLambda_{ii} \vu_0 + \nonumber \\
& 2\sumAllPointsi \vu_0\tran \barMQ_{0i} \vu_i + \sumAllPointsi \vu_i\tran (\barMQ_{ii}+\barLambda_{ii})\vu_i \\
& \hspace{-13mm}= \sum\limits_{i=1}^N \underbrace{ \vu_0\tran (-\barLambda_{ii})\vu_0 + \vu_0\tran (2 \barMQ_{0i})\vu_i + \vu_i\tran (\barMQ_{ii}+\barLambda_{ii})\vu_i}_{m_i}.
\eea
Further denoting $\vu_i = [\barvu_i\tran\ u_i]\tran$ with $\barvu_i \in \Real{3}$, $m_i$ can be written as:
\bea
& m_i = \bmat{c}
\barvu_0 \\ u_0
\emat\tran \bmat{cc}
-\ME_{ii} & \zero \\
\zero & \frac{\barcsq}{4}
\emat 
\bmat{c}
\barvu_0 \\ u_0
\emat + \nonumber \\
& \bmat{c}
\barvu_0 \\ u_0
\emat\tran 
\bmat{c|c}
\substack{ \left( \Vert \va_i \Vert^2 - \frac{\barcsq}{2} \right)\eye_3 \\ -\vSkew{\va_i}^2 - \va_i \va_i\tran } & \MZero \\
\hline
\MZero & - \frac{\barcsq}{2} 
\emat
\bmat{c}
\barvu_i \\ u_i
\emat + \nonumber \\
& \bmat{c}
\barvu_i \\ u_i
\emat\tran
\bmat{c|c}
\substack{ \left( \Vert \va_i \Vert^2 + \frac{\barcsq}{2} \right)\eye_3 \\ - \vSkew{\va_i}^2 - \va_i \va_i\tran + \ME_{ii}} & \MZero \\
\hline
\MZero & \frac{\barcsq}{4}
\emat
\bmat{c}
\barvu_i \\ u_i
\emat \\
& = \frac{\barcsq}{4}\underbrace{ \left( u_0^2 - 2u_0 u_i + u_i^2\right)}_{=(u_0-u_i)^2 \geq 0}+ \barvu_0\tran (-\ME_{ii}) \barvu_0 +  \nonumber \\
&\barvu_0\tran \left( \Vert \va_i \Vert^2 \eye_3 - \frac{\barcsq}{2}\eye_3 - \vSkew{\va_i}^2 - \va_i\va_i\tran \right) \barvu_i + \nonumber \\
& \hspace{-5mm}\barvu_i\tran \left(\Vert \va_i \Vert^2\eye_3 + \frac{\barcsq}{2} \eye_3 - \vSkew{\va_i}^2 - \va_i \va_i\tran + \ME_{ii} \right) \barvu_i, \label{eq:isolateScalar}
\eea
where equality holds only when $u_i=u_0$ in the underbraced inequality in~\eqref{eq:isolateScalar}. Now we insert the choice of $\ME_{ii}$ in eq.~\eqref{eq:choiceOfE} to $m_i$ to get the following inequality:
\bea
& m_i \geq \barvu_0\tran (-\vSkew{\va_i}^2)\barvu_0  + \frac{1}{4} \barcsq \barvu_0\tran \barvu_0 + \nonumber \\
& \hspace{-8mm}\Vert \va_i \Vert^2 \barvu_0\tran \barvu_i - \frac{\barcsq}{2}\barvu_0\tran \barvu_i + \barvu_0\tran (-\vSkew{\va_i}^2) \barvu_i - \barvu_0\tran \va_i \va_i\tran \barvu_i + \nonumber \\
&  \Vert \va_i \Vert^2 \barvu_i\tran \barvu_i + \frac{1}{4} \barcsq \barvu_i\tran \barvu_i - \barvu_i\tran \va_i \va_i\tran \barvu_i. \label{eq:afterInsertingEii}
\eea
Using the following facts:
\bea
& \Vert \va_i \Vert^2 \barvu_0\tran \barvu_i = \barvu_0\tran (-\vSkew{\va_i}^2 + \va_i\va_i\tran) \barvu_i; \\
& \Vert \va_i \Vert^2 \barvu_i\tran \barvu_i = \barvu_i\tran (-\vSkew{\va_i}^2 + \va_i\va_i\tran) \barvu_i, 
\eea
eq.~\eqref{eq:afterInsertingEii} can be simplified as:
\bea
& m_i \geq \barvu_0\tran (-\vSkew{\va_i}^2)\barvu_0  + \frac{1}{4} \barcsq \barvu_0\tran \barvu_0 + \nonumber \\
& 2\barvu_0\tran (-\vSkew{\va_i}^2)\barvu_i - \frac{\barcsq}{2} \barvu_0\tran \barvu_i + \nonumber \\
& \barvu_i\tran (-\vSkew{\va_i}^2) \barvu_i + \frac{1}{4} \barcsq \barvu_i\tran \barvu_i \\
& = \left( \vSkew{\va_i} \barvu_0 + \vSkew{\va_i} \barvu_i \right)\tran \left( \vSkew{\va_i} \barvu_0 + \vSkew{\va_i} \barvu_i \right) + \nonumber \\
&  \frac{\barcsq}{4} \left( \barvu_0\tran \barvu_0 - 2\barvu_0\tran \barvu_i  + \barvu_i\tran \barvu_i \right) \\
& = \Vert \va_i \times (\barvu_0 + \barvu_i) \Vert^2 +  \frac{ \barcsq}{4} \Vert  \barvu_0 -  \barvu_i \Vert^2  \nonumber \\
& \geq 0.
\eea
Since each $m_i$ is nonnegative, $\vu\tran \MN^\star \vu \geq 0$ holds true for any vector $\vu$ and therefore $\MN^\star \succeq 0$ is true. To see $\MN^\star$ only has one zero eigenvalue, we notice that $\vu\tran \MN^\star \vu = 0$ holds only when:
\bea
\begin{cases} \label{eq:zeroConditions}
u_i = u_0, \forall i=1,\dots,N \\
% \Vert \barvu_i \Vert^2 = 0, \forall i=1,\dots,N \\
\barvu_0=\barvu_i, \forall i=1,\dots,N \\
\va_i \times (\barvu_0 + \barvu_i) = \zero_3,\forall i=1,\dots,N
\end{cases}
\eea
because we have more than two $\va_i$'s that are not parallel to each other, eq.~\eqref{eq:zeroConditions} leads to $\barvu_0=\barvu_i = \zero_3,\forall i=1,\dots,N$. Therefore the only set of nonzero vectors that satisfy the above conditions are $\{\vu \in \Real{4(N+1)}: \vu = a\vr,a\in\Real{} \text{ and }a\neq 0\}$. Therefore, $\MN^\star$ has only one zero eigenvalue and $\rank{\MN^\star}=4(N+1)-1$.
\end{proof} 
Proposition~\ref{prop:constructionDualVariable} indeed proves the original Theorem~\ref{thm:strongDualityNoiseless} by giving valid constructions of dual variables under which strong duality always holds in the noiseless and outlier-free case.
\end{proof}

==> sections/quaternionEstimation.tex <==
%!TEX root = ../main.tex

\subsection{Robust Rotation Estimation: The Quaternion Case}
\label{sec:quaternionEstimation}


We now adopt a quaternion formulation for~\eqref{eq:TLSWahbaRot}. 
 Quaternions are an alternative representation for 3D rotations~\cite{Shuster93jas-attitude,Breckenridge99tr-quaternions} and their use will simplify the derivation of our 
 convex relaxation in Section~\ref{sec:SDPRelaxation}. We start by reviewing basic facts about quaternions and then state the quaternion-based \TWlong formulation in Problem~\ref{prob:qTW} below.  


{\bf Preliminaries on Unit Quaternions.}
% Since we will formulate the robust Wahba problem using unit quaternion representation, we provide brief preliminaries of unit quaternion that will be used in the following sections. 
We denote a unit quaternion as a unit-norm column vector $\vq=[\vv\tran\ s]\tran$, where $\vv \in \Real{3}$ is the \emph{vector part} of the quaternion and the last element $s$ is the \emph{scalar part}. We  also use $\vq = [q_1\ q_2\ q_3\ q_4]\tran$ to denote the four entries of the quaternion. 

Each quaternion represents a 3D rotation and the composition of two rotations $\vq_a$ and $\vq_b$ can be 
computed using the \emph{quaternion product} $\vq_c = \vq_a \kron \vq_b$:
\bea \label{eq:quatProduct}
\vq_c = \vq_a \kron \vq_b = \MOmega_1(\vq_a) \vq_b = \MOmega_2(\vq_b) \vq_a,
\eea
where $\MOmega_1(\vq)$ and $\MOmega_2(\vq)$ are defined as follows:
% If we define two linear mappings $\MOmega_1(\vq)$ and $\MOmega_2(\vq)$ that each maps a vector in $\Real{4}$ to a matrix in $\Real{4\times4}$ as:
\vspace{-3mm}
\begin{equation} \label{eq:Omega_1}
\arraycolsep=2pt\def\arraystretch{0.5}
\scriptscriptstyle \MOmega_1(\vq) \scriptscriptstyle = 
\scriptscriptstyle \left[ \scriptscriptstyle \begin{array}{cccc}
\scriptscriptstyle q_4 & \scriptscriptstyle -q_3 &  \scriptscriptstyle q_2 &  \scriptscriptstyle q_1 \\
\scriptscriptstyle q_3 & \scriptscriptstyle q_4 & \scriptscriptstyle -q_1 & \scriptscriptstyle q_2 \\
\scriptscriptstyle -q_2 & \scriptscriptstyle q_1 & \scriptscriptstyle q_4 & \scriptscriptstyle q_3 \\
\scriptscriptstyle -q_1 & \scriptscriptstyle -q_2 & \scriptscriptstyle -q_3 & \scriptscriptstyle q_4 
\scriptscriptstyle \end{array} \scriptscriptstyle \right],\quad 
\arraycolsep=2pt\def\arraystretch{0.5}
\scriptscriptstyle \MOmega_2(\vq) = \scriptscriptstyle
\bmat{cccc}
\scriptscriptstyle q_4 & \scriptscriptstyle q_3 & \scriptscriptstyle -q_2 & \scriptscriptstyle q_1 \\
\scriptscriptstyle -q_3 & \scriptscriptstyle q_4 & \scriptscriptstyle q_1 & \scriptscriptstyle q_2 \\
\scriptscriptstyle q_2 & \scriptscriptstyle -q_1 & \scriptscriptstyle q_4 & \scriptscriptstyle q_3 \\
\scriptscriptstyle -q_1 & \scriptscriptstyle -q_2 & \scriptscriptstyle -q_3 & \scriptscriptstyle q_4 
\emat.
\end{equation}
\vspace{-3mm}
The inverse of a quaternion $\vq=[\vv\tran\ s]\tran$ is defined as:
%is straightforward and can be done by reversing the sign of the vector part:
\bea
\label{eq:q_inverse}
\vq\inv = \bmat{c}
-\vv \\
s
\emat,
\eea
where one simply reverses the sign of the vector part. 
% \red{Using~\eqref{eq:q_inverse}, one can verify that the following equalities hold:
% \bea \label{eq:OmegaofInverse}
% \MOmega_1(\vq\inv) = \MOmega_1\tran(\vq),\quad \MOmega_2(\vq\inv) = \MOmega_2\tran(\vq).
% \eea}

The rotation of a vector $\va \in \Real{3}$ can be expressed in terms of quaternion product. 
Formally, if $\MR$ is the (unique)  rotation matrix corresponding to a unit quaternion $\vq$, then:
\bea
\label{eq:q_pointRot}
\bmat{c}
\MR \va \\
0 
\emat = \vq \kron \hat{\va} \kron \vq\inv,
\eea
where $\hat{\va}=[\va\tran\ 0]\tran$ is the homogenization of $\va$, obtained by augmenting $\va$ with an extra entry equal to zero.

The set of unit quaternions, denoted as $\sphere{3}=\{\vq\in\Real{4}: \Vert \vq \Vert = 1\}$, is the \emph{3-Sphere} manifold.  $\sphere{3}$ is a \emph{double cover} of $\SOthree$ since $\vq$ and $-\vq$ represent the same rotation (intuitively, eq.~\eqref{eq:q_pointRot} implements the same rotation if we replace $\vq$ with $-\vq$, since the matrices in~\eqref{eq:Omega_1} are linear in $\vq$).
% that contains the set of all unit-norm vectors in $\Real{4}$ (unit quaternions)


{\bf Quaternion-based Robust Wahba Problem.}
Equipped with the relations reviewed above, it is now easy to rewrite~\eqref{eq:TLSWahbaRot}  
using unit quaternions. 

\begin{problem}[Quaternion-based Robust Wahba]\label{prob:qTW}
 The robust Wahba problem~\eqref{eq:TLSWahbaRot} can be equivalently written as: %using unit quaternions as:
%
\bea \label{eq:TLSWahba} 
\min_{\vq \in \sphere{3}}  \sumAllPointsi \min \left( \frac{1}{\betaNoise_i^2} \Vert \hatvb_i - \vq \otimes \hatva_i \otimes \vq\inv \Vert^2 \;,\; \barcsq \right),
\eea
% where $\sphere{3}=\{\vq\in\Real{4}: \Vert \vq \Vert = 1\}$ is the \emph{3-Sphere} manifold that contains the set of all unit-norm vectors in $\Real{4}$ (unit quaternions), 
where we defined 
$\hatva_i \doteq [\va_i\tran \; 0]\tran$ and $\hatvb_i \doteq [\vb_i\tran \; 0]\tran$, and 
$\otimes$ denotes the quaternion product.  
%the fact that $\vq \otimes \hatva_i \otimes \vq\inv$ performs a rotation of the vector $\va_i$.
\end{problem}

The equivalence between~\eqref{eq:TLSWahba} and~\eqref{eq:TLSWahbaRot} can be easily understood from eq.~\eqref{eq:q_pointRot}.
The main advantage of using~\eqref{eq:TLSWahba} is that we replaced the set \SOthree with a simpler set, the set of unit-norm vectors $\sphere{3}$. 
%However, the simpler, but still non-convex norm constraint


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Binary Cloning and \QCQP}
\label{sec:binaryClone}

The goal of this section is to rewrite~\eqref{eq:TLSWahba} as a Quadratically-Constrained Quadratic Program (\QCQP). We do so in three steps: (i) we show that~\eqref{eq:TLSWahba} can be written using binary variables, (ii) we show that the problem with binary variables can be written using $N+1$ quaternions, and (iii) we manipulate the resulting problem to expose its quadratic nature. The derivation of the \QCQP will pave the way to our convex relaxation (Section~\ref{sec:SDPRelaxation}).
%the cost can be written as a quadratic function. 


{\bf From Truncated Least Squares to Mixed-Integer Programming.}
Problem~\eqref{eq:TLSWahba} is hard to solve globally, due to the non-convexity of both the cost function and  the constraint ($\sphere{3}$ is a non-convex set). As a first re-parametrization, we expose the non-convexity of the cost by 
rewriting the \TLS cost using binary variables. 
% The first technique we use is to introduce binary variables to write the cost function in additive form. 
Towards this goal, we rewrite the inner ``$\min$'' in~\eqref{eq:TLSWahba} using the following property, that holds for any pair of  scalars $x$ and $y$: 
%write the minimum of two real scalars $a$ and $b$ as a minimization over a binary variable $\theta$:
\bea
\label{eq:minxy}
\min(x,y)=\min_{\theta \in \{+1,-1\}} \frac{1+\theta}{2}x + \frac{1-\theta}{2}y.
\eea
Eq.~\eqref{eq:minxy} can be verified to be true by inspection: the right-hand-side returns $x$ (with minimizer $\theta=+1$) 
if $x<y$, and $y$ (with minimizer $\theta=-1$) if $x>y$. This enables us to rewrite problem \eqref{eq:TLSWahba} as a mixed-integer program including the quaternion
$\vq$ and binary variables $\theta_i, \; i=1,\ldots,N$:
%
\bea \label{eq:TLSadditiveForm}
\min_{\substack{ \vq \in S^3 \\ \theta_i = \{\pm1\}} } \sumAllPointsi \frac{1+\theta_i}{2}\frac{\Vert \hatvb_i - \vq \kron \hatva_i \kron \vq\inv \Vert^2}{\betaNoise_i^2}  + \frac{1-\theta_i}{2}\barcsq.
\eea
%
The reformulation is related to the Black-Rangarajan duality 
between robust estimation and line processes~\cite{Black96ijcv-unification}: the \TLS cost is an extreme case of robust function that results in a binary line process.
Intuitively, the binary variables $\{\theta_i\}_{i=1}^N$ in problem~\eqref{eq:TLSadditiveForm} decide whether a given measurement $i$ is an inlier 
($\theta_i=+1$) or an outlier ($\theta_i=-1$).
% inform the inlier or outlier set membership of the corresponding pair of measurements: $(\va_i, \vb_i)$ is a pair of inliers if $\theta_i=+1$, and outliers if $\theta_i=-1$.

{\bf From Mixed-Integer to Quaternions.}
Now we convert the mixed-integer program~\eqref{eq:TLSadditiveForm} to an optimization over $N+1$ quaternions. The intuition is that, if we define extra quaternions $\vq_i \doteq \theta_i \vq$, 
we can rewrite~\eqref{eq:TLSadditiveForm} as a function of $\vq$ and $\vq_i$ ($i=1,\ldots,N$). This is a key step towards getting a quadratic cost (Proposition~\ref{prop:qcqp}). 
The re-parametrization is formalized in the following proposition.
\vspace{-2mm}
\begin{proposition}[Binary cloning] \label{prop:binaryCloning}
The mixed-integer program~\eqref{eq:TLSadditiveForm} is equivalent (in the sense that they admit the same 
optimal solution $\vq$) to the following optimization
%
% \begin{align} \label{eq:TLSadditiveForm2}
% \min_{\substack{ \vq \in S^3 \\ \vq_i = \{\pm\vq\}} } & 
% \sumAllPointsi \frac{\Vert \hatvb_i - \vq \kron \hatva_i \kron \vq\inv \Vert^2}{2\betaNoise_i^2} +\\
% &+  \frac{\Vert \vq\tran\vq_i \hatvb_i - \vq \kron \hatva_i \kron \vq_i\inv \Vert^2}{2\betaNoise_i^2} 
% + \frac{1-\vq\tran\vq_i}{2}\barcsq 
% \end{align}
% \begin{align} 
\bea
\label{eq:TLSadditiveForm2}
\min_{\substack{ \vq \in S^3 \\ \vq_i = \{\pm\vq\}} } & \hspace{-4mm}
\displaystyle\sumAllPointsi 
\displaystyle\frac{\Vert \hatvb_i \!-\! \vq \kron \hatva_i \kron \vq\inv 
+ \vq\tran\vq_i \hatvb_i \!-\! \vq \kron \hatva_i \kron \vq_i\inv \Vert^2  
}{4\betaNoise_i^2} \nonumber \hspace{-5mm}\\
&\displaystyle  + \frac{1-\vq\tran\vq_i}{2}\barcsq.   \hspace{-5mm}
\eea
% \end{align}
%
which involves $N+1$ quaternions ($\vq$ and $\vq_i$, $i=1,\ldots,N$).
\end{proposition}
While a formal proof is given in the \supp, it is fairly easy to see that 
if $\vq_i = \{\pm\vq\}$, or equivalently, $\vq_i = \theta_i \vq$ with $\theta_i \in \{\pm1\}$, then 
$\vq_i\tran\vq = \theta_i$, and $\vq \kron \hatva_i \kron \vq_i\inv =  \theta_i ( \vq \kron \hatva_i \kron \vq\inv)$ which exposes the relation between~\eqref{eq:TLSadditiveForm}  and~\eqref{eq:TLSadditiveForm2}.  
We dubbed the re-parametrization~\eqref{eq:TLSadditiveForm2} \emph{binary cloning} since now we created a ``clone'' $\vq_i$ for each measurement, such that $\vq_i = \vq$ for inliers (recall that $\vq_i = \theta_i \vq$) and $\vq_i = -\vq$ for outliers.


{\bf From Quaternions to \QCQP.}
We conclude this section by showing that~\eqref{eq:TLSadditiveForm2} can be actually written as a \QCQP. 
% We then use the binary variables $\{\theta_i\}_{i=1}^N$ to make $N$ copies of the unit quaternion $\vq$: $\{\vq_i \doteq \theta_i \vq \}_{i=1}^N$ and conveniently reformulate problem (\ref{eq:TLSadditiveForm}) as a \emph{quadratically constrained quadratic program} (QCQP).
This observation is non-trivial since~\eqref{eq:TLSadditiveForm2} has a \emph{quartic} cost and $\vq_i = \{\pm\vq\}$ 
is not in the form of a quadratic constraint. 
The re-formulation as a \QCQP is given in the following.
\vspace{-2mm}
\begin{proposition}[Binary Cloning as a \QCQP] \label{prop:qcqp}
Define a single column vector $\vxx = [\vq\tran\ \vq_1\tran\ \dots\ \vq_N\tran]\tran$ 
stacking all variables in Problem~\eqref{eq:TLSadditiveForm2}. 
Then, Problem~\eqref{eq:TLSadditiveForm2}  
is equivalent (in the sense that they admit the same 
optimal solution $\vq$) to the following Quadratically-Constrained Quadratic Program:
\beal \label{eq:TLSBinaryClone}
%\hspace{-8mm} %\substack{\min \\ \vq,\vq_i} 
\displaystyle\min_{\vxx \in \Real{4(N+1)}} & \sum\limits_{i=1}^N \vxx\tran \MQ_i \vxx \\
\subject &  \vxx_q\tran \vxx_q = 1 \hspace{30mm} \\
& \vxx_{q_i} \vxx_{q_i}\tran = \vxx_{q} \vxx_{q}\tran, \forall i = 1,\dots,N %\nonumber 
\eeal
where $\MQ_i \in \Real{4(N+1)\times 4(N+1)}$ ($i=1,\ldots,N$) are known symmetric matrices that depend on the 3D vectors $\va_i$ and 
$\vb_i$ (the explicit expression is given in the \supp), and the notation $\vxx_q$ (resp. $\vxx_{q_i}$) denotes the 4D subvector of $\vxx$ corresponding to $\vq$ (resp. $\vq_i$).
\end{proposition}

A complete proof of Proposition~\ref{prop:qcqp} is given in the \supp.
 Intuitively, (i) we developed the squares in the cost function~\eqref{eq:TLSadditiveForm2}, (ii) we used the properties of unit quaternions (Section~\ref{sec:TLSFormulation}) to simplify the expression to a quadratic cost, and (iii) we adopted the 
 more compact notation afforded by the vector $\vxx$ to obtain~\eqref{eq:TLSBinaryClone}. 
 % \red{Moreover, we noticed that for a unit quaternion $\vq$, the equality $\vq_i \vq_i\tran = \vq \vq\tran$ holds if and only if $\vq_i \in \{\pm\vq\}$.}
 % Intuitively, we developed the squares in the cost function~\eqref{eq:TLSadditiveForm2} and used the properties of unit quaternions (Section~\ref{sec:TLSFormulation}) to simplify the expression to a quadratic cost. \red{Moreover, we noticed that for a unit quaternion $\vq$, the equality $\vq_i \vq_i\tran = \vq \vq\tran$ holds if and only if $\vq_i \in \{\pm\vq\}$.}



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Semidefinite Relaxation}
\label{sec:SDPRelaxation}
Problem~\eqref{eq:TLSBinaryClone} writes the \TWlong problem as a \QCQP. 
Problem~\eqref{eq:TLSBinaryClone} is still a non-convex problem (quadratic equality constraints are non-convex).
% but now the non-convexity is confined to the constraints, while the cost is convex. 
Here we develop a convex semidefinite programming (SDP) relaxation for problem~\eqref{eq:TLSBinaryClone}. 

The crux of the relaxation consists in rewriting problem~\eqref{eq:TLSBinaryClone}  
% is that if we concatenate all quaternions $\vq$ and $\{\vq_i\}_{i=1}^N$ 
% into a single column vector $\vxx = [\vq\tran\ \vq_1\tran\ \dots\ \vq_N\tran]\tran$, then 
% Problem~\eqref{eq:TLSBinaryClone} can be written 
as a function of the following matrix:
% consists in noticing that we can write Problem~\eqref{eq:TLSBinaryClone} as 
% a function of the following matrix. 
% Let us concatnate all the decision variables $\vq$ and $\{\vq_i\}_{i=1}^N$ in a single column vector $\MX = [\vq\tran\ \vq_1\tran\ \dots\ \vq_N\tran]\tran$, and we observe the lifted version of $\MX$, $\MZ \doteq \MX\tran \MX$ contains all linear and quadratic terms in $\vq$ and $\vq_i$:
\bea \label{eq:matrixZ}
\MZ = \vxx \vxx\tran = \bmat{cccc}
\vq\vq\tran & \vq \vq_1\tran & \cdots & \vq\vq_N\tran \\
\star & \vq_1\vq_1\tran & \cdots & \vq_1\vq_N\tran \\
\vdots & \vdots & \ddots & \vdots \\
\star & \star & \cdots & \vq_N \vq_N\tran 
\emat.
\eea
% In particular, we can write~\eqref{eq:TLSBinaryClone} as:
% %
%  \bea \label{eq:with_x}
% \min_{\vxx} & \trace{\vxx\tran \MQ \vxx} \\
% \subject & \vxx\tran \ME_1 \vxx = 1 \nonumber \\
% & \vxx\tran \ME_{i+1} \vxx = \vxx\tran \ME_1 \vxx, \\
% & \forall i=1,\dots,N \nonumber
% \eea
For this purpose we note that if we define $\MQ \doteq \sum_{i=1}^N \MQ_i$:
\beal
\sum\limits_{i=1}^N \vxx\tran \MQ_i \vxx = \vxx\tran \MQ \vxx = %\trace{\vxx\tran \MQ \vxx} = 
\trace{ \MQ \vxx \vxx\tran} = \trace{\MQ \MZ}
\eeal
and that $\vxx_{q_i} \vxx_{q_i}\tran = [\MZ]_{q_i q_i}$, where  
$[\MZ]_{q_i q_i}$ denotes the $4\times4$ diagonal block of $\MZ$ with row and column indices corresponding to $\vq_i$.
Since any matrix in the form $\MZ = \vxx \vxx\tran$ is a positive-semidefinite rank-1 matrix, we obtain:
\vspace{-2mm}
\begin{proposition}[Matrix Formulation of Binary Cloning] \label{prop:qcqpZ}
Problem~\eqref{eq:TLSBinaryClone}
is equivalent (in the sense that optimal solutions of a problem can be mapped to optimal solutions of the other) 
to the following non-convex program:
\bea \label{eq:qcqpZ}
\min_{\MZ \succeq 0} & \trace{\MQ \MZ} \nonumber \\
\subject & \trace{[\MZ]_{qq}} = 1 \nonumber \\
& [\MZ]_{q_i q_i} = [\MZ]_{qq}, \;\; \forall i=1,\dots,N \nonumber \\
& \rank{\MZ} = 1
\eea
% where $\MQ_i \in \Real{4(N+1)\times 4(N+1)}$ are known symmetric matrices that depend on the 3D vectors $\va_i$ and 
% $\vb_i$ (the explicit expression is given in the supplemental), and the notation $\vxx_q$ (resp. $\vxx_{q_i}$) denotes the 4D subvector of $\vxx$ corresponding to $\vq$ (resp. $\vq_i$).
\end{proposition}
\vspace{-2mm}
At this point it is straightforward to  develop a (standard) SDP relaxation 
by dropping the rank-1 constraint, which is the only source of non-convexity in~\eqref{eq:qcqpZ}.
% We first provide a naive relaxation (the ) 
\vspace{-2mm}
\begin{proposition}[Naive SDP Relaxation] \label{prop:naiveRelax}
The following SDP is a convex relaxation of Problem~\eqref{eq:qcqpZ}:
\bea \label{eq:naiveRelaxation}
\min_{\MZ \succeq 0}  & \trace{\MQ \MZ} \\
\subject  & \trace{[\MZ]_{qq}} = 1 \nonumber \\
& [\MZ]_{q_i q_i} = [\MZ]_{qq}, \forall i=1,\dots,N \nonumber
\eea
% where $\MQ$ is a known matrix (complete expression given in the supplementary), and 
% $[\MZ]_{q_i q_i}$ denote the $4\times4$ diagonal block of $\MZ$ with row and column indices corresponding $\vq_i$. 
\end{proposition}

% It is easy to check optimality 
% \begin{proposition}[Certification of Optimality]\label{prop:certification}
% When there is no noise and no outliers in the measurements, the SDP relaxation in \eqref{eq:naiveRelaxation} is always tight, meaning that:
% \begin{enumerate}
% \item the optimal cost of~\eqref{eq:naiveRelaxation} matches the optimal cost of the \QCQP~\eqref{eq:TLSBinaryClone},
% \item the optimal solution $\MZ^\star$ of~\eqref{eq:naiveRelaxation} is such that $\rank{\MZ^\star}=1$, and 
% \item $\MZ^\star$ can be written as $\MZ^\star = (\vxx^\star) (\vxx^\star)\tran$ where $\vxx^\star \doteq [(\vq^\star)\tran \; (\vq_1^\star)\tran \; \ldots \; (\vq_N^\star)\tran]$ is a global minimizer of the original non-convex problem~\eqref{eq:TLSBinaryClone}.
% \end{enumerate}
% \end{proposition}
The following theorem proves that the naive SDP relaxation~\eqref{prop:naiveRelax} 
is tight in the absence of noise and outliers.

\begin{theorem}[Tightness in Noiseless and Outlier-free Wahba]\label{thm:strongDualityNoiseless}
When there is no noise and no outliers in the measurements, and there are at least two vector measurements ($\va_i$'s) that are \edit{not parallel} to each other, the SDP relaxation~\eqref{eq:naiveRelaxation} is always \emph{tight}, \ie:
\begin{enumerate}
\item the optimal cost of~\eqref{eq:naiveRelaxation} matches the optimal cost of the \QCQP~\eqref{eq:TLSBinaryClone},
\item the optimal solution $\MZ^\star$ of~\eqref{eq:naiveRelaxation} has rank 1, and 
\item $\MZ^\star$ can be written as $\MZ^\star = (\vxx^\star) (\vxx^\star)\tran$ where $\vxx^\star \doteq [(\vq^\star)\tran \; (\vq_1^\star)\tran \; \ldots \; (\vq_N^\star)\tran]$ is a global minimizer of the original non-convex problem~\eqref{eq:TLSBinaryClone}.
\end{enumerate}
\end{theorem}

A formal proof, based on Lagrangian duality theory, is given in the \supp. While Theorem~\ref{thm:strongDualityNoiseless} ensures that the naive SDP relaxation computes optimal solutions in noiseless and outlier-free problems, our original motivation was to solve problems with many outliers. 
One can still empirically assess tightness by solving the SDP and verifying if a rank-1 solution is obtained.
Unfortunately, the naive relaxation produces solutions with rank larger than 1 in the presence of outliers, \cf~Fig.~\ref{fig:naiveRelaxation}(a).
Even when the rank is larger than 1, one can \emph{round} the solution by computing a rank-1 approximation of 
$\MZ^\star$; however, we empirically observe that, whenever the rank is larger than 1, the 
rounded estimates exhibit large errors, as shown in Fig.~\ref{fig:naiveRelaxation}(b).

To address these issues, we propose to add \emph{redundant constraints} to \emph{tighten} (improve) the SDP relaxation, \edit{inspired by~\cite{Briales17cvpr-registration,Tron15rssws3D-dualityPGO3D}}.
The \edit{following} proposed relaxation
% , presented in the proposition below, 
is tight (empirically satisfies the three claims of Theorem~\ref{thm:strongDualityNoiseless}) even in the presence of noise and \maxOutliers of outliers.
% However, as we will show in Section~\ref{sec:experiments}, the naive relaxation in (\ref{eq:naiveRelaxation}) quickly fails when there are outliers in the measurements. Hence, we draw insights from recent results of successfully using \emph{redundant constraints} to \emph{tighten} (improve) SDP relaxation~\cite{Briales18cvpr-global2view,Briales17cvpr-registration,nesterov2000handbook-sdpRelaxation}, and propose the following convex relaxation with redundant constraints.
\begin{proposition}[SDP Relaxation with Redundant Constraints] \label{prop:relaxationRedundant}
The following SDP is a convex relaxation of~\eqref{eq:qcqpZ}:
\bea \label{eq:relaxationRedundant}
\min_{\MZ \succeq 0} & \trace{\MQ \MZ} \label{eq:SDPrelax} \\
\subject %& \MZ \succeq 0 \nonumber \\
& \trace{[\MZ]_{qq}} = 1 \nonumber \\
& [\MZ]_{q_i q_i} = [\MZ]_{qq}, \forall i=1,\dots,N \nonumber \\
& [\MZ]_{q q_i} = [\MZ]\tran_{q q_i}, \forall i=1,\dots,N \nonumber \\
& [\MZ]_{q_i q_j} = [\MZ]\tran_{q_i q_j}, \forall 1\leq i < j \leq N \nonumber
\eea
and it is always tighter, \ie the optimal objective  of~\eqref{eq:SDPrelax} is always closer to the optimal objective of~\eqref{eq:TLSBinaryClone}, when compared to the naive relaxation~\eqref{eq:naiveRelaxation}.
\end{proposition}

We name the improved relaxation~\eqref{eq:SDPrelax} \name (\nameLong).
While our current theoretical results only guarantee  tightness  in the noiseless and outlier-free case (Theorem~\ref{thm:strongDualityNoiseless} also holds for \name, since it is always tighter than the naive relaxation), 
in the next section we empirically demonstrate the tightness of~\eqref{eq:SDPrelax} 
in the face of noise and extreme outlier rates, \cf~Fig.~\ref{fig:naiveRelaxation}.


==> sections/result-benchmarkBnB.tex <==
%!TEX root = main.tex

\section{Benchmark against \bnb}
\label{sec:benchmarkBnB}
\edit{We follow the same experimental setup as in Section~\ref{sec:exp_synthetic} of the main document, and benchmark \name against (i) \emph{Guaranteed Outlier Removal}~\cite{Bustos2015iccv-gore3D} (label: \GORE); (ii) \bnb with \emph{L-2 distance threshold}~\cite{bazin2012accv-globalRotSearch} (label: \BnBLtwo); and (iii) \bnb with \emph{angular distance threshold}~\cite{Bustos2015iccv-gore3D} (label: \BnBAng). Fig.~\ref{fig:benchmarkBnBGORE} boxplots the distribution of rotation errors for 30 Monte Carlo runs in different combinations of outlier rates and noise corruptions. In the case of low inlier noise ($\sigma=0.01$), \name is robust against $96\%$ outliers and achieves significantly better estimation accuracy compared to \GORE, \BnBLtwo and \BnBAng, all of which experience failures at $96\%$ outlier rates (Fig.~\ref{fig:benchmarkBnBGORE}(a,b)). In the case of high inlier noise ($\sigma=0.1$), \name is still robust against $80\%$ outlier rates and has lower estimation error compared to the other methods. }

\input{fig-benchmarkBnBGORE}


==> sections/result-imageStitching.tex <==
%!TEX root = main.tex

\section{Image Stitching Results}
\label{sec:imageStitching}
Here we provide extra image stitching results. As mentioned in the main document, we use the \emph{Lunch Room} images from the PASSTA dataset~\cite{meneghetti2015scia-PASSATImageStitchingData}, which contains 72 images in total. We performed pairwise image stitching for 12 times, stitching image pairs $(6i+1,6i+7)$ for $i=0,\dots,11$ (when $i=11$, $6i+7=73$ is cycled to image 1). The reason for not doing image stitching between consecutive image pairs is to reduce the relative overlapping area
 so that \SURF~\cite{Bay06eccv} feature matching is more prone to output outliers, 
 creating a more challenging benchmark for \name.
 % This way, we create a more challenging test for \name.
 
 \name successfully performed all 12 image stitching tasks and Table~\ref{tab:imageStitchingStatistics} reports the statistics. 
%
As we mentioned in the main document, the stitching of image pair (7,13) was the most challenging, due to the high outlier ratio of $66\%$, and the \ransac-based stitching method~\cite{Torr00cviu,Hartley04book} as implemented by the Matlab ``\scenario{estimateGeometricTransform}'' function failed in that case. We show the failed example from \ransac in Fig.~\ref{fig:failedRansac}.

\input{tab-imageStitchStatistics}
\input{fig-ransacfail}

==> sections/rotationEstimation.tex <==
%!TEX root = ../main.tex





==> sections/rotationMatrixEstimation.tex <==
%!TEX root = ../main.tex


\subsection{Robust Rotation Estimation: The Rotation Matrix Case}
 \label{sec:rotationEstimation}

% In this section we use the translation invariant measurements in eq.~\eqref{eq:TIM} and the scale estimate $\hats$ from Algorithm~\ref{alg:adaptiveVoting}
%  to 
% estimate the orthogonal matrix $\MR$. 
The generative model~\eqref{eq:TIM} describes measurements $\TIMb_{ij}$ affected 
by bounded noise $\| \veps_{ij} \| \leq \beta_{ij}$ including potential outliers (when $\vo_{ij} \neq \bm{0}$).
Again, we estimate $\MR$ from the estimated scale $\hats$, the measurements $\TIMb_{ij}$ and the bounds $\beta_{ij}$ using a 
\TLS estimator:
\bea
\label{eq:TLSrotation}
\hatMR = \argmin_{\MR \in \Othree} \sumAllIM \min
\left( \frac{  \|  \TIMb_k - \hats \MR \TIMa_k \|^2 }{  \beta^2_k }  
\;,\; 
\barcsq \right)
\eea
where for simplicity we numbered the measurements from $1$ to $K = |\calE|$ and adopted the notation $\TIMa_k, \TIMb_{k}$ instead of $\TIMa_{ij}, \TIMb_{ij}$. \edit{We have also relaxed $\MR \in \SOthree$ to $\MR \in \Othree$, where $\Othree \doteq \setdef{\MR\in\Real{3 \times 3}}{\MR\tran \MR = \eye_3}$ is the \emph{Orthogonal Group}, which includes proper rotations and reflections. } For simplicity of notation, in the following we drop $\hats$ and assume that \edit{$\TIMa_1,\ldots,\TIMa_K$} have been corrected by the scale ($\TIMa_k \leftarrow \hats \TIMa_k$).

% Clearly, the machinery developed in Section~\ref{sec:scaleEstimation} only applies to the scalar case, while~\eqref{eq:TLSrotation} is intractable in general, since it requires optimizing a non-convex cost (the \TLS is non-convex) over a non-convex domain ($\Othree$).

A fundamental contribution of this paper is to develop a tight convex relaxation for~\eqref{eq:TLSrotation}. The relaxation is tight even in presence of a large number (\maxOutliersRot) of outliers and provides per-instance suboptimality guarantees. %\todo{add guarantees}.
% We develop our convex relaxation below. 
Before presenting the relaxation, we  
introduce a binary formulation that is instrumental to develop the proposed relaxation.
%that facilitates the development of the convex relaxation.

\myParagraph{Binary formulation and \nameCloning} 
The first insight behind our convex relaxation is the fact that we can write the \TLS cost~\eqref{eq:TLSrotation} in additive form using auxiliary binary variables (a property recently leveraged in a different context by~\cite{Lajoie19ral-DCGM}): 
\bea
\label{eq:TLSrotation2}
\min_{
\substack{\MR \in \Othree,\\
\theta_k \in\{-1,+1\}, \forall k }} % k=1,\ldots,\nrTIM} 
\sumAllIM 
\frac{ (1 + \theta_k) }{ 2 } \frac{  \|  \TIMb_k -  \MR \TIMa_k \|^2 }{  \beta^2_k }  
+ 
\frac{ (1 - \theta_k) }{ 2 } 
\barcsq 
\eea
%
The equivalence can be easily understood from the fact that $\min(x,y)=\min_{\theta \in\{-1,+1\}} 
\frac{ (1 + \theta ) }{ 2 } x + \frac{ (1 - \theta) }{ 2 } y$.
% for instance, when $x<y$, the minimization will prefer $\theta=+1$ that leads to an optimal cost of $x$, while $\theta=-1$ is preferred for $x>y$. 

We conveniently rewrite~\eqref{eq:TLSrotation2} by replacing the binary variables with suitable (orthogonal) matrices. 
\begin{proposition}[\nameCloning]\label{prop:cloning}
Problem~\eqref{eq:TLSrotation2}
is equivalent to the following optimization problem
\bea
\hspace{-3mm}
\min_{
\substack{\MR, \MR_k, \forall k }} % 
\!\!&
\!\!\sumAllIM 
\frac{  \| \TIMb_k - \MR \TIMa_k 
+ \MR\tran \MR_k  \TIMb_k - \MR_k \TIMa_k \|^2 }{ 4 \beta^2_k }  
+ 
\frac{ (1 - \ve_1\tran \MR\tran \MR_k \ve_1) }{ 2 } 
\barcsq \hspace{-5mm} \nonumber 
\\
\subject 
\hspace{-7mm}&
\MR\tran\MR=\eye_3, \;\; \MR_k\tran\MR_k=\eye_3,
\nonumber 
 \\
& \MR\tran\MR_k \in\{-\eye,+\eye\},
\; k=1,\ldots,\nrTIM \hspace{-5mm}\label{eq:TLSrotation4}
\eea
where we introduced a matrix $\MR_k \in \Real{3\times3}$ for each $k=1,\ldots,\nrTIM$, and defined the vector $\ve_1 \doteq [1 \; 0 \; 0]\tran$. 
\end{proposition}

A formal proof of~\prettyref{prop:cloning} is given in the \supp. 
% Intuitively, 
% we made the constraint $\MR \in \Othree$ explicit as $\MR\tran\MR=\eye_3$; more importantly,
% we replaced the scalar variable $\theta_k \in \{-1,+1\}$ 
% with matrix variables $\MR_k \in \{-\MR,+\MR\}$ (the ``binary'' nature of $\MR_k$ is enforced by the constraints). Indeed, from the objective of~\eqref{eq:TLSrotation4}, it is easy to see that when $\MR_k = \MR$ the $k$-th term in the objective becomes $\frac{  \| \TIMb_k - \MR \TIMa_k \|^2 }{ \beta^2_k }$ ($k$ is treated as an inlier, similarly to choosing $\theta_k=+1$), while when $\MR_k = -\MR$ the $k$-th term is equal to $\barcsq$ ($k$ is treated as an outlier, similarly to choosing $\theta_k=-1$).
 We name the re-parametrization in~\prettyref{prop:cloning} \emph{binary cloning}, since we now have $\nrTIM$ clones of $\MR$ 
 (namely $\MR_k=\theta_k \MR \in \{\MR,-\MR\}$, $k=1,\ldots,\nrTIM$) that 
 are in charge of rejecting outliers: when $\MR_k = \MR$ the $k$-th term in the objective becomes $\frac{  \| \TIMb_k - \MR \TIMa_k \|^2 }{ \beta^2_k }$ (i.e., $k$ is treated as an inlier, similarly to choosing $\theta_k=+1$), while when $\MR_k = -\MR$ the $k$-th term is equal to $\barcsq$ (i.e., $k$ is treated as an outlier, similarly to choosing $\theta_k=-1$).
This reparametrization enables our relaxation.

\myParagraph{Convex relaxation} 
% We are now ready to introduce 
The proposed relaxation  is presented in~\prettyref{prop:TLSrotationRelax}. 
The main goal of this paragraph is to provide the intuition behind our relaxation, while the interested 
reader can find a formal derivation in the \supp. 

Let us define a $3 \times 3(\nrTIM+2)$ matrix $\MX = [\eye_3 \; \MR \; \MR_1 \; \ldots \; \MR_\nrTIM]$, stacking all unknown variables in~\eqref{eq:TLSrotation4}. We observe that the matrix $\MZ \doteq \MX\tran \MX$ contains all linear and quadratic terms in $\MR$ and $\MR_k$:
\bea
\label{eq:Z}
\MZ \doteq\MX\tran \MX  = 
\begin{array}{ccccccc}
\hspace{-4mm}\overbrace{}^{I} \hspace{1mm} \overbrace{}^{R} \hspace{1mm} \overbrace{}^{R_1} \hspace{5mm} \ldots \hspace{5mm}  \overbrace{}^{R_\nrTIM}  \\
% & R & R_1 & \ldots & R_\nrTIM  \\
\left[
\begin{array}{ccccccc}
\eye_3 & \MR & \MR_1 & \ldots & \MR_\nrTIM \\
\star &   \eye_3   &  \MR\tran\MR_1     &   \ldots     &      \MR\tran\MR_\nrTIM       \\
\star &    \star        &  \eye_3            &   \ldots     &        \MR_1\tran\MR_\nrTIM     \\
\star &    \vdots        &  \vdots         &   \ddots     &    \vdots        \\
\star &    \star        &  \star   &     \ldots    &    \eye_3        
\end{array}
\right]
\end{array}
\eea
Now it is easy to see that the cost function in~\eqref{eq:TLSrotation4} can be rewritten as a function  of $\MZ$, by 
noting that $\MR, \MR\tran \MR_k, \MR_k$ (appearing in the cost) are entries of $\MZ$, see~\eqref{eq:Z}. 
The constraints in~\eqref{eq:TLSrotation4} can be similarly written as a function of $\MZ$. For instance, 
the constraints $\MR\tran\MR=\eye_3$ and $\MR_k\tran\MR_k=\eye_3$ simply enforce that the block diagonal entries of $\MZ$ are identity matrices. Similarly, $\MR\tran\MR_k \in\{-\eye,+\eye\}$ can be rewritten as a (non-convex) constraint involving off-diagonal entries of $\MZ$.
Finally, the fact that $\MZ \doteq \MX\tran \MX$ implies $\MZ$ is positive semidefinite and has rank $3$ (number of rows in $\MX$, see~\eqref{eq:Z}).

According to the discussion so far, we can reparametrize problem~\eqref{eq:TLSrotation4} 
 using $\MZ$, and we can then develop a convex relaxation by relaxing all the resulting non-convex constraints.
 This is formalized in the following proposition.

\begin{proposition}[\TLS Rotation Estimation: Convex Relaxation]\label{prop:TLSrotationRelax}
The following convex program is a relaxation of~\eqref{eq:TLSrotation4}:  
\bea
\min_{
\substack{\MZ \succeq 0}} % 
& \hspace{-5mm} \trace{\barMQ \MZ} \hspace{-3mm}\label{eq:TLSrotationRelax}
\\
\subject 
& \hspace{-5mm} [\MZ]_{RR} =\eye_3, 
\;\;\; [\MZ]_{R_k R_k} =\eye_3,
\;\;\; [\MZ]_{II} =\eye_3,
\nonumber \hspace{-3mm}
 \\
& \hspace{-5mm} [\MZ]_{RR_k} = (\ve_1\tran [\MZ]_{RR_k} \ve_1) \eye_3, \;\; \forall k \nonumber \hspace{-3mm}\\
%|| R - Ri || <= 1 - trace(R'Ri)/3
& \hspace{-5mm} \|  [\MZ]_{IR} \pm [\MZ]_{IR_k} \| \leq  1 \pm (\ve_1\tran [\MZ]_{RR_k} \ve_1), \;\; \forall k \nonumber \hspace{-3mm}\\
%|| Ri - Rj || <= 1 - trace(Rj'Rj)/3
& \hspace{-5mm} \|  [\MZ]_{IR_k} \pm [\MZ]_{IR_{k'}} \| \leq  1 \pm (\ve_1\tran [\MZ]_{R_k R_{k'}} \ve_1), \;\; \forall k,k' \nonumber \hspace{-3mm}
\eea
where $\bar\MQ$ is a known $3(\nrTIM+2) \times 3(\nrTIM+2)$ symmetric matrix (expression given in the supplementary), 
and $[\MZ]_{RR_k}$ denotes a $3\times3$ block of $\MZ$ whose row indices correspond to the location of $\MR$ in $\MX$ (\cf with indices at the top of the matrix in eq.~\eqref{eq:Z})
and column indices correspond to the location of $\MR_k$ in $\MX$ (similarly, for $[\MZ]_{RR}$, $[\MZ]_{R_k R_k}$, $[\MZ]_{II}$, etc.). 
\end{proposition}
% \myParagraph{Per-instance guarantees}

The convex program~\eqref{eq:TLSrotationRelax} can be solved in polynomial time using off-the-shelf convex solvers, such 
as \cvx~\cite{CVXwebsite}. It is a relaxation, in the sense that the set of feasible solutions of~\eqref{eq:TLSrotationRelax} 
includes the set of feasible solutions of~\eqref{eq:TLSrotation4}. 
Moreover, it enjoys the typical per-instance guarantees of convex relaxations.

\begin{proposition}[Guarantees for \TLS Rotation Estimation]\label{prop:TLSrotation}
Let $\MZ^\star$ be the optimal solution of the relaxation~\eqref{eq:TLSrotationRelax}.
If $\MZ^\star$ has rank 3, then it can be factored as $\MZ^\star = (\MX^\star)\tran(\MX^\star)$, where $\MX^\star \!\doteq\! [\eye_3, {\MR}^\star, {\MR}^\star_1,\mydots, {\MR}^\star_\nrTIM]$ is the first block row of $\MZ^\star$. Moreover,  ${\MR}^\star, {\MR}^\star_1,\mydots, {\MR}^\star_\nrTIM$ is an optimal solution for~\eqref{eq:TLSrotation4}.
 % Moreover, let us call $\hat{\MX} \doteq [\eye_3, \hat{\MR}, \hat{\MR}_1,\ldots, \hat{\MR}_\nrTIM]$ the \emph{rounded estimate} obtained by projecting the entries $[\MZ\star]_{II}, [\MZ\star]_{IR}, [\MZ\star]_{IR_1}, \ldots, [\MZ\star]_{IR_\nrTIM}$ of $\MZ^\star$ to \Othree (\cf with the first row of~\eqref{eq:Z}).
% Let $f_R^\circ$ be the optimal objective of the convex relaxation~\eqref{eq:TLSrotationRelax},
% $f_R^\star$ be the optimal objective of~\eqref{eq:TLSrotation4}, and
%   $\hat{f}_R$ the objective attained in~\eqref{eq:TLSrotation4} by the rounded estimate $\hat{\MX}$.
%   Then, $f_R^\circ \leq f_R^\star \leq \hat{f}_R$  
% The optimal objective of the convex relaxation~\eqref{eq:TLSrotationRelax} is a lower bound for the optimal solution of the 
\end{proposition}

Empirically, we found that our relaxation is tight (i.e., \edit{numerically} produces a rank-3 solution) even when \maxOutliersRot of the \TIMs are outliers. 
 Even when the relaxation is not tight, one can still project $\MZ^\star$ to a feasible solution of~\eqref{eq:TLSrotation4} 
and obtain an upper-bound on how suboptimal the resulting solution is. 

In summary, the function ${\tt estimate\_R}$ in Algorithm~\ref{alg:ITR} solves the convex program~\eqref{eq:TLSrotationRelax} 
(e.g., using \cvx) to obtain a matrix $\MZ^\star$ and extracts the rotation estimate $\hatMR$ from $\MZ^\star$. 
In particular,  $\hatMR = [\MZ^\star]_{IR}$ if $\MZ^\star$ has rank 3 (\prettyref{prop:TLSrotation}), or $\hatMR$ is computed as the projection of 
$[\MZ^\star]_{IR}$ to \Othree otherwise.
%, when the rank of $\MZ^\star$ is larger 
% We note that our relaxation heavily relies on the geometry of the orthogonal matrices involved in~\eqref{eq:TLSrotation4} (the presence of the orthogonality constraints is key to making the relaxation tight).
% Indeed, one of the insights of this paper is that we should treat rotation estimation in a radically different manner, with respect to 
% robust estimation in vector spaces.
%robust rotation registration offers 
%insight is that we should treat rotation and vector spaces differently

==> sections/scaleEstimation_old.tex <==
%!TEX root = main.tex

\subsection{Robust Scale Estimation}
\label{sec:scaleEstimation}

In this section we use the rotation and translation invariant measurements in eq.~\eqref{eq:TRIM} to 
estimate the scale $s$. The generative model~\eqref{eq:TRIM} describes measurements $s_{ij}$ affected 
by bounded noise $|\eps^s_{ij}| \leq \alpha_{ij}$ including potential outliers (when $o^s_{ij} \neq 0$).
Again, we estimate the scale given the measurements $s_{ij}$ and the bounds $\alpha_{ij}$ using a 
\TLS estimator:
\bea
\label{eq:TLSscale}
\hats = \argmin_{s} \sumAllIM \min\left( \frac{  (  s-s_k )^2 }{  \alpha^2_k }  \;,\; \barcsq \right)
\eea
where for simplicity we numbered the measurements from $1$ to $K = |\calE|$ and adopted the notation $s_k$ instead of $s_{ij}$.
% From the previous section we have a bunch of measurements of the scale, potentially affected by outliers:
% \bea
% s_k \doteq \frac{  \|  \vb_{ij} \| }{  \|  \va_{ij} \| }  = s + \hat{o}_{ij} 
% \eea
% \TLS estimator:
% %
% \bea
% \label{eq:TLSscale}
% % s^\star = \argmin_{s} \sumAllPoints \min\left( (s - s_k)^2 , \barcsq \right)
% s^\star = \argmin_{s,\theta_k \in \{-1,+1\}} 
% \sumAllPoints \frac{(1+\theta_k)}{2}  \frac{(s - s_k)^2}{\sigma_s^2}  + \frac{(1-\theta_k)}{2}  \barcsq 
% \eea

The following theorem relates the \TLS estimator~\eqref{eq:TLSscale} to \emph{consensus maximization}, 
a popular framework for robust estimation in vision~\cite{Speciale17cvpr-consensusMaximization,Liu18eccv-registration}. 
This is instrumental to design a polynomial-time solution for~\eqref{eq:TLSscale} (\prettyref{thm:maxConsensusAlgo}). 

\begin{theorem}[\TLS Scale Estimation]\label{thm:scalarTLS}
Whenever the consensus set is unique, the optimal solution $\hats$ of the \TLS scale estimation~\eqref{eq:TLSscale} can be computed in two steps:
\begin{enumerate}
\item Consensus maximization: %Find the maximum consensus set: 
\beq
\label{eq:consensusMax}
(z^\star, \calS^\star) = \argmax_z \sumAllPoints \calI\left( \frac{(z - s_k)}{\alpha_k^2} \leq \barcsq \right)
\eeq
where $\calI$ is the indicator function, which is $1$ when the argument is true and zero otherwise.
Problem~\eqref{eq:consensusMax} returns a (typically non unique) $z^\star$ and a consensus set $\calS^\star$ 
that are such that $\frac{(z^\star - s_k)}{\alpha_k^2} \leq \barcsq$ for all $k\in \calS^\star$.
\item Least squares scale estimation over the consensus set: 
\beq
\hats = \left(\sum_{k\in \calS^\star } \frac{1}{\alpha_k^2}\right)\inv  \sum_{k\in \calS^\star} \frac{1}{\alpha_k^2} s_k
\eeq
\end{enumerate}
\end{theorem}
% consensus maximization is a popular framework~\cite{Speciale17cvpr-consensusMaximization,Liu18eccv-registration}, 
A proof of~\prettyref{thm:scalarTLS} is  given in Appendix~\ref{sec:proof:scalarTLS}.

While~\prettyref{thm:scalarTLS} draws an interesting connection between two robust estimation frameworks, 
it appear not to provide a tractable algorithmic solution, since exact consensus maximization~\cite{Speciale17cvpr-consensusMaximization,Liu18eccv-registration} is intractable in general. 
Our insight here is that, while consensus maximization is hard in general, it can be solved in polynomial time in the 
scalar case. 

An intuition is given in Fig.~\ref{fig:consensusMax},  
% ========================
\input{fig-consensusMax} 
% ========================

Problem~\eqref{eq:consensusMax} can be solved exactly using the adaptive voting scheme described in Algorithm~\ref{alg:adaptiveVoting}.

\begin{algorithm}[h]
\SetAlgoLined
\textbf{Input:} \ $s_k, \beta_k$\; 
\textbf{Output:} \  $(\calS^\star,y^\star)$, where the maximum consensus set $\calS^\star$  and $y^\star$ solve the consensus maximization~\eqref{eq:consensusMax}\;
\% Define vector and sort \\
\indent $\vv = [s_1 - \beta_1, s_1 + \beta_1,\ldots,s_\nrPoints - \beta_\nrPoints, s_\nrPoints + \beta_\nrPoints]$ \\
\indent $\vv = \text{sort}(\vv)$ \\
\% Compute middle points \\%\;
\For{$i = 1,\ldots,2\nrPoints-1$}{$m_i = \frac{\vv_{2i-1} + \vv_{2i}}{2}$}
 \% Voting \\%\;
 \For{$i = 1,\ldots,2\nrPoints-1$}{
 	$\calS_i = \emptyset$\\
 	\For{$k = 1,\ldots,\nrPoints$}{
		\If{$m_i \in [s_k - \beta_k, s_k + \beta_k]$}{
			$\calS_i = \calS_i \cup \{k\}$ \% add to consensus set\\
		}
	}
}
\% Pick largest consensus set\\
$i^\star = \argmax_i |\calS_i|$\\
 \textbf{return:} $(\calS_i, m_i)$ 
 % \While{g(S) > R}{
 %  $S_{i+1} \leftarrow S_i \cup \{ \underset{a \in G \backslash S_i}{\text{arg min}} \ {\rm{MG}}_g(a | S_i)  \}$ \;
 % }
 \caption{Adaptive Voting.\label{alg:adaptiveVoting}}
\end{algorithm} 


\begin{theorem}[Optimality of Algorithm~\ref{alg:adaptiveVoting}]\label{thm:maxConsensusAlgo}
Algorithm~\ref{alg:adaptiveVoting} computes an optimal solution for Problem~\eqref{eq:consensusMax} 
in $\calO(K^2)$.
\end{theorem}

Proof is given in Appendix~\ref{sec:proof:maxConsensusAlgo}.


estimate must be positive: convex combination of positive quantities

==> sections/table-objectPoseEstimation.tex <==
%!TEX root = ../main.tex

\begin{table}[h!]
\centering
\begin{tabular}{ccccc}
& \shortstack{Rotation \\ error [rad]} & \shortstack{Translation \\ error [m]} & \shortstack{\# of FPFH \\ correspondences} &\shortstack{FPFH inlier \\ ratio [\%]} \\
\hline
Mean & 0.066 & 0.069 & 525 & 6.53 \\
\hline
SD & 0.043 & 0.053 & 161 & 4.59\\
\hline
\end{tabular}
\caption{Registration results \red{on eight scenes} of the RGB-D dataset~\cite{Lai11icra-largeRGBD}.}
\label{tab:objectPoseEstimation}
\end{table}

==> sections/translationEstimation.tex <==
%!TEX root = main.tex

\subsection{Robust Translation Estimation}
\label{sec:translationEstimation}
% After obtaining an estimate of the scale $\hats$ and the rotation $\hatMR$, we can substitute them into the original formulation~\eqref{eq:TLSRegistration} and solve the resulting optimization problem to compute an estimate of the translation $\vt$. 
%
Since we already presented a polynomial-time solution for scalar \TLS in \prettyref{sec:scaleEstimation}, we propose to solve 
for the translation component-wise, i.e., 
% Unfortunately, While the \TLS problem can be solved efficiently in the scalar case (\prettyref{sec:scaleEstimation}), 
% it is hard to solve in the multi-variate case. 
%
% In this paper, we propose a simple but effective approximation: rather than computing $\vt$ from solving~\eqref{eq:TLSRegistration} 
% (with given $\hats$, $\hatMR$), 
we compute the entries $t_1, t_2, t_3$ of $\vt$ independently (see the \supp\ for details): 
% as the minimizers of: 
% %
 \bea
 \label{eq:TLSRegistrationT1}
 \min_{ \substack{ t_j } } 
 \sumAllPointsi \min \left( \frac{1}{\beta_i^2} \left|  [\vb_i - \hats \hatMR \va_i]_j - t_j \right|^2 \!\!,  \barcsq \right), \;\; j=1,2,3
 \eea
 where $[\cdot]_j$ denotes the $j$-th entry of a vector. %Note that $t_j$ is the only unknown in~\eqref{eq:TLSRegistrationT1}.
%  %Note that $\vb_i - \hats \hatMR \va_i$ are known vectors
% % This formulation is related to the optimization of  
% % Note that~\eqref{eq:TLSRegistrationT1} enforces that the estimated  
% While the solution to~\eqref{eq:TLSRegistrationT1} will not match in general the solution to~\eqref{eq:TLSRegistration}, 
% problem~\eqref{eq:TLSRegistrationT1} 
% %is also designed 
% also has the effect
% to bound the maximum admissible error for each inlier measurement 
% to $\beta_i$, but while~\eqref{eq:TLSRegistration} operates on the $\ell_2$ norm of the vector, operates component-wise~\eqref{eq:TLSRegistrationT1} (in other words, while the error in our original noise model was confined within the $\ell_2$-norm ball,
% it has been now relaxed to the $\ell_\infty$-norm ball). % (i.e., as an $\ell_\infty$ norm).  

% we can transform point cloud $\calA$ by $\hats$ and $\hatMR$, and subtract it from point cloud $\calB$:
% \bea
% \vb_i - \hats \hatMR \va_i = \vt + \veps_i + \vo_i
% \eea
% Because the three coordinates of $\vt$ can be considered mutually independant, we can use the same adaptive voting algorithm in the scalar case to solve the three coordinates of $\vt$ separately and assemble them together using data $\{\vb_i, \hats \hatMR \va_i \}$.

In summary, the function ${\tt estimate\_t}$ in Algorithm~\ref{alg:ITR} calls Algorithm~\ref{alg:adaptiveVoting} three times 
(one for each entry of $\vt$) and returns the translation estimate $\hatvt = [t_1\;t_2\;t_3]$. 
% and then computes the largest maximum clique in the resulting graph. All measurements that do not belong to the clique are 
% rejected as outliers.
% In conclusion, the function ${\tt estimate\_R}$ in Algorithm~\ref{alg:ITR} solves the convex program~\eqref{eq:TLSrotationRelax} 
% (e.g., using \cvx) to obtain a matrix $\MZ^\star$ and extracts the rotation estimate $\hatMR$ from $\MZ^\star$. 
% In particular,  $\hatMR = [\MZ^\star]_{IR}$ if $\MZ^\star$ has rank 3 (\prettyref{prop:TLSrotation}), or $\hatMR$ is computed as the projection of 
% $[\MZ^\star]_{IR}$ to \Othree otherwise.
